Making Higher Order MOT Scalable: An Efficient Approximate Solver for Lifted Disjoint Paths

We present an efficient approximate message passing solver for the lifted disjoint paths problem (LDP), a natural but NP-hard model for multiple object tracking (MOT). Our tracker scales to very large instances that come from long and crowded MOT sequences. Our approximate solver enables us to process the MOT15/16/17 benchmarks without sacrificing solution quality and allows for solving MOT20, which has been out of reach up to now for LDP solvers due to its size and complexity. On all these four standard MOT benchmarks we achieve performance comparable or better than current state-of-the-art methods including a tracker based on an optimal LDP solver.

==> idf1_plot.tex <==
\begin{tikzpicture}[scale=0.9]
\begin{axis}[
    title={IDF1 Ours vs. Lif\_T},
    width=0.5\textwidth,
    height=0.3\textwidth,
    xlabel={\text{Sequence length} [frames]},
    ylabel={IDF1},
    ymin=0.7, ymax=0.9,
    xmin=0, xmax=200,
    xtick={0,30,50,75,100, 125, 150,200},
    ytick={0.7,0.8,0.9},
    legend pos=north west,
    ymajorgrids=true,
    grid style=dashed,
    log ticks with fixed point,
    x tick label style={/pgf/number format/1000 sep=\,},
    legend style={at={(0.42,0.18)},anchor=west},
    legend columns=2
]

\addplot[
    color=green,
    mark=square,
    ]
    coordinates {
    (30,0.852)(50,0.833)(75,0.826)(100,0.825)(150,0.81)(200,0.754)
    };

\addplot[
    color=blue,
    mark=square,
    ]
    coordinates {
    (30,0.852)(50,0.833)(75,0.826)(100,0.825)(150,0.81)(200,0.754)
    };

\addplot[
    color=orange,
    mark=square,
    ]
    coordinates {
    (30,0.852)(50,0.815)(75,0.816)(100,0.816)(150,0.798)(200,0.746)

    };

\addplot[
    color=red,
    mark=square,
    ]
    coordinates {
    (30,0.846)(50,0.806)(75,0.794)(100,0.804)(150,0.781)(200,0.732)
    };
    \legend{Ours-6,Ours-11,Ours-31, Gurobi}
    
\end{axis}
\end{tikzpicture}

==> lifted disjoint paths message passing/Lagrange-decomposition.tex <==
\section{Lagrange Decomposition Algorithm for LDP}
\label{sec:Lagrange-decomposition}
Below we recapitulate  
Lagrange decomposition and the message passing primitive used in our algorithm (Sec.~\ref{sec:lagrange-decomposition-sub}).
Then, we propose a decomposition of the LDP problem~\eqref{eq:lifted-disjoint-paths-problem} into smaller but tractable subproblems (Sec.~\ref{sec:inout-subproblems}-\ref{sec:cut-subproblem}).
This decomposition is a dual task to an LP-relaxation of~\eqref{eq:lifted-disjoint-paths-problem}. Therefore, it provides a~lower bound that is iteratively increased by the message passing. We solve Problem~\eqref{eq:lifted-disjoint-paths-problem} in a simplified version of Lagrange decomposition framework developed in~\cite{Swoboda_2017_CVPR}.
Our heuristic for obtaining primal solutions uses the dual costs from the subproblems (Sec.~\ref{sec:primal-rounding}).
% The dual costs from the subproblems are used in our heuristic for obtaining primal solutions (Section~\ref{sec:primal-rounding}).
\subsection{Lagrange Decomposition}
\label{sec:lagrange-decomposition-sub}
We have an optimization problem $\min_{x \in \mathcal{X}} \langle c, x \rangle$ where $\mathcal{X}\subseteq \{0,1\}^n$ is a feasible set and $c\in \mathbb{R}^n$ is the objective vector. Its Lagrange decomposition is given by 
a~set of \emph{subproblems} 
$\mathcal{S}$
with associated \emph{feasible sets} 
$\mathcal{X}^{\mathsf{s}}\subseteq \{0,1\}^{d_\mathsf{s}}$ for each $\mathsf{s}\in \mathcal{S}$. 
Each coordinate $i$ of $\mathcal{X}^{\mathsf{s}}$ corresponds to one coordinate  of $\mathcal{X}$ via an injection $\pi_{\mathsf{s}}:[d_{\mathsf{s}}]\rightarrow [n]$
alternatively represented by a matrix
$A^{\mathsf{s}}\in \{0,1\}^{d_{\mathsf{s},n}}$ where $(A^{\mathsf{s}})_{ij}=1\Leftrightarrow \pi_\mathsf{s}(i)=j$.
%We denote the image of $\pi_{s}$ as $\img(\pi_s) = \{\pi_s(i): i \in [d_s]\}$.
% Moreover, $A_{\mathsf{s}}\in \{0,1\}^{d_{\mathsf{s}},n}$ defines selection of subproblem coordinates $ (A_{\mathsf{s}})_{ij}=1\Leftrightarrow \pi_\mathsf{s}(i)=j$.
For each pair of subproblems $\mathsf{s},\mathsf{s'}\in \mathcal{S}$ that contain a pair of coordinates $i,j$ such that $\pi_{\mathsf{s}}(i)=\pi_{\mathsf{s'}}(j)$, we have a~\emph{coupling constraint} $x^\mathsf{s}_i = x^{\mathsf{s}'}_j$ for each  $x^\mathsf{s} \in \mathcal{X}^\mathsf{s}$, $x^{\mathsf{s}'} \in \mathcal{X}^{\mathsf{s}'}$.


We require that every feasible solution $x\in \mathcal{X}$ is feasible for the subproblems, i.e.\ $\forall x\in \mathcal{X},\forall \mathsf{s}\in \mathcal{S}: A^{\mathsf{s}}x \in \mathcal{X}^s$. 


We require that the objectives of subproblems are equivalent to the original objective, i.e.\ 
$\la c, x \ra = \sum_{s \in \mathcal{S}} \la \theta^s, A^{\mathsf{s}}x \rangle$ $\forall x \in \mathcal{X}$. Here, $\theta^\mathsf{s} \in \R^{d_{\mathsf{s}}}$ defines the \emph{objective} of subproblem $\mathsf{s}$.

The \emph{lower bound} of the Lagrange decomposition given the costs $\theta^{\mathsf{s}}$ for each $\mathsf{s}\in \mathcal{S}$ is 
\begin{equation}
\label{eq:lower-bound}
    \sum_{\mathsf{s} \in \mathcal{S}} \min_{x^\mathsf{s} \in \mathcal{X}^\mathsf{s}} \la \theta^\mathsf{s}, x^\mathsf{s} \ra\,.
\end{equation}

Given coupling constraint $x^\mathsf{s}_i = x^{\mathsf{s}'}_j$  and $\gamma \in \R$, a  sequence of operations of the form
$ \theta^\mathsf{s}_i \pluseq \gamma,\ \theta^{\mathsf{s}'}_j \minuseq \gamma$ is called a~\emph{reparametrization}.



% \begin{definition}[Lagrange decomposition]
% A Lagrange decomposition is given by a set of \emph{subproblems} 
% $\mathcal{S}$
% with associated \emph{feasible sets} 
% $\mathcal{X}^{\mathsf{s}}\subseteq \{0,1\}^{\abs{X^\mathsf{s}}}$ for each $ \mathsf{s} \in \mathcal{S}$ and
% \emph{coupling constraints} $\mathcal{C}^{\mathsf{s},\mathsf{s}'}$ for pairs of subproblems $\mathsf{s},\mathsf{s}' \in \mathcal{S}$ constraining $x^\mathsf{s} \in \mathcal{X}^\mathsf{s}, x^{\mathsf{s}'} \in \mathcal{X}^{\mathsf{s}'}$  to  $x^\mathsf{s}_i = x^{\mathsf{s}'}_j$ for all variable pairs $(i,j) \in \mathcal{C}^{\mathsf{s},\mathsf{s}'}$.
% For every subproblem an \emph{objective} is given by $\theta^\mathsf{s} \in \R^{\abs{\mathsf{s}}}$.
% Its \emph{lower bound} is given by
% \begin{equation}
% \label{eq:lower-bound}
%     \sum_{\mathsf{s} \in \mathcal{S}} \min_{x^\mathsf{s} \in \mathcal{X}^\mathsf{s}} \la \theta^\mathsf{s}, x^\mathsf{s} \ra\,.
% \end{equation}
% A sequence of operations of the form
% \begin{equation}
% \label{eq:reparametrization}
%     \theta^\mathsf{s}_i \pluseq \gamma,\quad 
%     \theta^{\mathsf{s}'}_j \minuseq \gamma
% \end{equation}
% for coupling constraint $x^\mathsf{s}_i = x^{\mathsf{s}'}_j$  and $\gamma \in \R$ is called a \emph{reparametrization}.
% \end{definition}
Feasible primal solutions are invariant under reparametrizations but the lower bound~\eqref{eq:lower-bound} is not.
%Below, we will explore reparametrization updates that are monotonically non-decreasing in the lower bound.
The optimum of the dual lower bound equals to the optimum of a convex relaxation of the original problem, see~\cite{guignard1987lagrangean}.

\myparagraph{Min-marginal message passing.}
Below, we describe reparametrization updates monotonically non-decreasing in the lower bound based on \emph{min-marginals}.
Given a variable $x^\mathsf{s}_i$ of a subproblem $\mathsf{s} \in  S$, the associated \emph{min-marginal} is
\begin{equation}
    \label{eq:min-marginal}
    m^{\mathsf{s}}_{i} =
    \min\limits_{x^\mathsf{s} \in \mathcal{X}^\mathsf{s}: x^\mathsf{s}_i = 1} \langle  \theta^{\mathsf{s}}, x^\mathsf{s} \rangle
    - \min\limits_{x^\mathsf{s} \in \mathcal{X}^\mathsf{s}: x^\mathsf{s}_i = 0} \langle  \theta^{\mathsf{s}}, x^\mathsf{s}  \rangle 
\end{equation}
i.e.\ the difference between the optimal solutions with the chosen variable set to $1$ resp.\ $0$.

\begin{proposition}[\cite{Swoboda_2017_CVPR}]
\label{prop:reparametrization}
Given a coupling constraints $x^\mathsf{s}_i = x^{\mathsf{s}'}_j$ and $\omega \in [0,1]$ the following operation is non-decreasing w.r.t.\ the dual lower bound~\eqref{eq:lower-bound}
    \begin{align}
        \label{eq:min-marginal-update}
        \theta^{\mathsf{s}}_{i} &\minuseq \omega \cdot m^{\mathsf{s}}_{i},& 
\theta^{\mathsf{s}'}_{j} &\pluseq \omega \cdot m^{\mathsf{s}}_{i}\,.
\end{align}

\end{proposition}

\myparagraph{The goal of reparametrization} is two-fold. 
(i)~Improving the objective lower bound to know how far our solution is from the optimum.
% (i) Obtaining the best possible lower bound of the objective function tells us how far our solution is from the optimum.
(ii)~Using reparametrized costs as the input for our primal heuristic yields high-quality primal solutions. The key components are efficient computations of (i)~optima of subproblems for obtaining lower bound~\eqref{eq:lower-bound}, (ii)~constrained optima for obtaining min-marginals \eqref{eq:min-marginal} and (iii)~a~primal heuristic using the reparametrized costs (Sec.~\ref{sec:primal-rounding}).
Lagrange decomposition has been used for other problems but the subproblem decomposition and minimization procedures are problem specific.
Therefore, developing them for LDP is an important contribution for solving LDP in a scalable way while keeping a~small gap to an optimum.
\subsection{Inflow and Outflow Subproblems}\label{sec:inout-subproblems}
For each node $v \in V$ of the flow graph, we introduce two subproblems:
An inflow and an outflow subproblem.
%one denoted by $x^{in}_v$ and $x^{out}_v$.
The subproblems contain all incoming resp.\ outgoing edges of node $v$ together with the corresponding node.
Formally, inflow resp.\ outflow subproblems contain the edges $ \delta^-_E(v) \cup \delta^-_{E'}(v)$, resp. $ \delta^+_E(w) \cup \delta^+_{E'}(w)\,.$
% \begin{align}
%     &\delta^+_E(v) \cup \delta^+_{E'}(v), & \delta^-_E(w) \cup \delta^-_{E'}(w)\,.
% \end{align}
Here, we adopt the standard notation where $\delta^-_E(v)$, resp.\ $\delta^+_E(v)$ denote all base edges incoming to $v$, resp. outgoing from $v$. 
Similarly, $\delta^-_{E'}(v), \delta^+_{E'}(v)$ denote lifted edges incoming to, resp.\ outgoing from $v$.

\myparagraph{The feasible set} $\mathcal{X}^{out}_v$ of the outflow subproblem for node $v$ is defined as
\begin{equation}
\label{eq:outflow-feasible-set}
    \left\{
\begin{array}{l}
   %(x,y,y') \in \{0,1\} \times \{0,1\}^{\delta^+_E(v)} \times \{0,1\}^{\delta^+_{E'}(v)} : \\
   z^{out}_v \in \{0,1\}, y^{out} \in \{0,1\}^{\delta^+_E(v)}, y'^{out} \in \{0,1\}^{\delta^+_{E'}(v)} : \\
   \ \ (z^{out}_v,y^{out},y'^{out}) = \mathbb{0}\ \vee \\
     \ \ \exists P \in vt\mhyphen\text{paths}(G) \text{ s.t. }
     \begin{array}[t]{c}
     z^{out}_v = 1 \\
     y^{out}_{vw} = 1 \Leftrightarrow vw \in P_E\\ 
     y'^{out}_{vu} = 1 \Leftrightarrow u \in P_V
     \end{array}
  \end{array}
    \right\}\,.
  \end{equation}
%The above constraints restrict the variables as follows:
Consequently, either there is no flow going through  vertex $v$ and all base and lifted edges
%adjacent to $v$
have label zero.
Alternatively, there exists a $vt\mhyphen$path $P$ in $G$ labeled by one.  
In this case the base edge adjacent to $v$ corresponding to the first edge in $P$ is one.
All lifted edges connecting $v$ with vertices of $P$ also have value one.
All other base and lifted edges are zero.
Each feasible solution of the outflow subproblem can be represented by a path $vt\mhyphen$path $P$.
The feasible set of the inflow subproblem  $\mathcal{X}^{in}_v$ is defined analogously.
We sometimes omit the  superscipts $out$ for better readability.

\myparagraph{Constraints between inflow and outflow subproblems.}
For node variables, we add the constraint $
    z^{in}_v = z^{out}_v$.
For an edge $vw \in E \cup E'$ we require the shared edge in the outflow subproblem of $v$ and in the inflow subproblem for $w$ to agree, i.e. $
        y_{vw}^{out} = y_{vw}^{in}$ if $vw \in E$ and  $    {y'}_{vw}^{out} = {y'}_{vw}^{in}$ if $vw \in E'$.



\myparagraph{Optimization of in- and outflow subproblems.} Given costs $\theta^{out}$, the optimal solution of an outflow problem for node $v$ can be computed by depth-first search on the subgraph defined by the vertices reachable from $v$.

\noindent The algorithms rely on the following data structures:
%\vspace{-\topsep}
\begin{itemize}
 %\setlength{\parskip}{0pt}
  %\setlength\itemsep{0pt}
    \item lifted\_costs$[u]$ contains the minimum cost of all $ut\mhyphen$paths w.r.t.\ to costs of all lifted edges connecting $v$ with the vertices of the path. 
    \item next$[u]$ contains the best neighbor of vertex $u$ w.r.t.\ values in lifted\_cost. That is, next$[u]=\argmin_{w:uw\in \delta^+_E(u)}\text{lifted\_cost}[w]$
\end{itemize}
\vspace{-\topsep}



\begin{algorithm}
 \caption{Opt-Out-Cost}  
 \label{alg:outflow-minimization}
 \textbf{Input} start vertex $v$, edge costs $\tilde{\theta}$\\
 \textbf{Output} optimal value $\mathrm{opt}$, $\text{lifted\_cost}$  $\forall w:vw \in \delta^+_E(v)$ optimal solution for $vw$ active $\alpha_{vw}$
    \begin{algorithmic}[1]
    \For{$u\in V:vu\in\mathcal{R}_{G}$}
    %\State $\text{lifted\_cost}[u] = \infty$, $\text{visited}[u] = false$, next$[u]=t$
    \State $\text{lifted\_cost}[u] = \infty$, next$[u]=\emptyset$
    \EndFor
    %\State$\text{lifted\_cost}[r] =0 $, $\text{visited}[r] = true$, next$[r]=t$
    \State$\text{lifted\_cost}[t] =0 $,  next$[t]=t$
    \State Lifted-Cost-DFS-Out($v,v,\tilde{\theta},\text{lifted\_cost},\text{next}$)
    \State $\forall w:vw \in \delta^+_E(v): \alpha_{vw} =  \tilde{\theta}_v + \tilde{\theta}_{vw} + \text{lifted\_cost}[w] $
    \State $\mathrm{opt} = \min(\min_{vw \in \delta^+_E(v)} \alpha_{vw}, 0)$
    % \State $opt' = \min_{w:vw \in \delta^+_E(v)} \tilde{\theta}_v + \tilde{\theta}_{vw} + \text{lifted\_cost}[w] $
    % \State $opt = \min(opt', 0)$
    \end{algorithmic}
\end{algorithm}
\roberto{To differentiate variables from functions other latex algorithm packages use the style \textbackslash texttt, for instance \texttt{Lifted-Cost-DFS}.}

\begin{algorithm}
\caption{Lifted-Cost-DFS-Out}
\label{alg:outflow-minimization-dfs}
 \textbf{Input} $v,u,\tilde{\theta},\text{lifted\_cost},\text{next}$\\
 \textbf{Output} $\text{lifted\_cost},\text{next}$
\begin{algorithmic}[1]
\State $\alpha=0$
\For{$uw \in \delta^+_{E}(u)$}
%\If{$\text{visited}[w] = false$}
\IIf{$\text{next}[w] = \emptyset$} Lifted-Cost-DFS-Out($v,w,\tilde{\theta}$)
\If{lifted\_cost$[w]<\alpha$}
%\State $m=\min \{\text{lifted\_cost}[w],m\}$
\State $\alpha=\text{lifted\_cost}[w]$, $\text{next}[u]=w$
\EndIf
\EndFor
\IIf{next$[u]=\emptyset$} next$[u]=t$ %\EndIIf
\State $\text{lifted\_cost}[u]=\alpha+\tilde{\theta}'_{vu}$
%\State $\text{visited}[u] = true$\;
\end{algorithmic}
\end{algorithm}

Alg.~\ref{alg:outflow-minimization} and~\ref{alg:outflow-minimization-dfs} give a general dept first search (DFS) procedure that, given a vertex $v$, computes optimal 
%Alg.~\ref{alg:outflow-minimization} and~\ref{alg:outflow-minimization-dfs} give a general DFS-procedure that, given a vertex $v$, computes optimal
paths from all vertices reachable from $v$.
Alg.~\ref{alg:outflow-minimization} takes as input vertex $v$ and edge costs $\tilde{\theta}$. Its subroutine Alg.~\ref{alg:outflow-minimization-dfs} computes recursively for each vertex $u$ reachable from $v$ the value  $\text{lifted\_cost}[u]$.
The overall optimal cost $\min_{(z,y,y') \in \mathcal{X}^{out}_v} \la \tilde{\theta}, (z,y,y') \rangle$ of the subproblem is given by the minimum of node and base edge and lifted edges costs $\min_{vu\in \delta^+_{E}(v)}\tilde{\theta}^{out}_v + \tilde{\theta}^{out}_{vu} + \text{lifted\_cost}[u]$.
We achieve linear complexity by exploiting that subpaths of minimum cost paths are minimal as well.
The optimization for the inflow subproblem is analogous.


\myparagraph{Message passing for in- and outflow subproblems.}
We could compute one min-marginal~\eqref{eq:min-marginal}  by adapting Alg.~\ref{alg:outflow-minimization} and forcing an edge to be taken or not.
However, computing min-marginals one-by-one with performing operation~\eqref{eq:min-marginal-update} would be inefficient, since it would involve calling Alg.~\ref{alg:outflow-minimization} $\mathcal{O}(\abs{\delta^+_E(v)} + \abs{\delta^+_{E'}(v))}$ times.
Therefore, we present efficient algorithms for computing a sequence of min-marginals in Appendix~\ref{sec:outflow-subproblem-min-marginals}.
The procedures save computations by choosing the order of edges for computing min-marginals suitably and reuse previous calculations.





\subsection{Path Subproblems}\label{sec:path-subproblem}
The subproblem contains a~lifted edge $vw$ and a~path $P$ from $v$ to $w$ consisting of both base and lifted edges. They reflect that 
(i)~lifted edge $vw$ must be labelled $1$ if there exists an active path between $v$ and $w$, and
(ii)~there cannot be exactly one inactive lifted edge within path $P$ if $vw$ is active. The reason is that the inactive lifted edge divides $P$ into two segments that must be disconnected. This is contradictory to activating lifted edge $vw$  because it indicates a connection between $v$ and $w$.
% Path subproblems reflect that 
% (i)~a lifted edge must be labelled $1$ if there exists an active path between the lifted edge's endpoints and
% (ii)~there cannot be exactly one inactive lifted edge within a path if the lifted edge between the first and the last vertex of the path is active.
Path subproblems are similar to cycle inequalities for the multicut~\cite{chopra1993partition}.
% A path subproblem is composed of a lifted edge $vw$ and a $vw\mhyphen$path $P$ consisting of both base and lifted edges. %in a union of the base graph and the lifted graph $G\cup G'=(V,E\cup E')$.

In order to distinguish between base and lifted edges of path $P$, we use notation $P_E=P\cap E$ and $P_{E'}=P\cap E'$. 
For the purpose of defining the feasible solutions of path subproblems, we define strong base edges $E_0=\{vw\in E|vw\mhyphen\text{paths}(G)=\{vw\}\}$.
That is, base edge $vw$ is strong iff there exists no other $vw\mhyphen$path in graph $G$ than  $vw$ itself.
\todo[inline]{Use $:$ instead of $|$ in the set?}
\andrea{I actually prefer $|$}
\roberto{Both are fine. I just meant to make it consistent. I saw sometimes $:$ and sometimes $|$, but may be this is gone now..}

\myparagraph{The feasible set} $\mathcal{X}^P$ of the path subproblem for $vw\mhyphen$path $P$ is defined as 
\begin{align}
\nonumber y\in &\{0,1\}^{P_E},y'\in \{0,1\}^{P_{E'}\cup\{ vw\}}:\\
\label{eq:path-subproblem-eq-lifted}
\forall& kl\in P_{E'}\cup \{vw\}: \\
\nonumber
&\sum_{ij\in P_E} (1-y_{ij})+\sum_{ij\in P_{E'}\cup \{vw\}\setminus \{kl\}} (1-y'_{ij})\geq 1-y'_{kl}\,,\\
\label{eq:path-subproblem-eq-strong}
\forall& kl\in P_{E}\cap E_0:\\ 
\nonumber &\sum_{ij\in P_E\setminus kl} (1-y_{ij})+\sum_{ij\in P_{E'}\cup \{vw\}} (1-y_{ij})\geq 1-y_{kl}\,. 
\end{align}

Equation~\eqref{eq:path-subproblem-eq-lifted} requires that a lifted edge in $P_{E'}$ or $vw$ can be zero only if at least one other edge of the subproblem is zero.
%The same holds true for all strong base edges, see
Equation~\eqref{eq:path-subproblem-eq-strong} enforces the same for strong base edges.



\myparagraph{The optimization of path subproblems } 
%The optimization of the path subproblem
is detailed in Alg.~\ref{alg:path-subproblem-optimization} in the Appendix. The principle is as follows.
It checks whether 
there exists exactly one positive edge and whether it is either a lifted or a strong base edge.
If so, the optimal solution is either 
(i)~all edges except the two largest ones or
(ii)~all edges, whichever gives smaller objective value.
If the above condition does not hold, the optimal solution can be chosen to contain all negative edges.

We use a~variation  of the path optimization algorithm with an edge fixed to $0$ or $1$ for computing min-marginals.
%A variation of the path optimization algorithm with an edge fixed to $0$ or $1$ is used for computing min-marginals



\myparagraph{Cutting plane.}
Since there are exponentially many path subproblems, we add during the optimization only those that improve the relaxation.
 Details are in Appendix~\ref{sec:cutting-planes-path-subproblems}.

\subsection{Cut Subproblems}\label{sec:cut-subproblem}
The purpose of a cut subproblem is to reflect that a lifted edge $uv$ must be labelled 0 if there exists a cut of base edges  that separate $u$ and $v$ ($uv\mhyphen$cut) all labelled $0$.

\myparagraph{The feasible set.}
A cut subproblem consists of a lifted edge $uv$ and a $uv\mhyphen$cut $C = \{ij \in E| i \in A, j \in B\}$ where $A,B \subset V$  with $A \cap B = \emptyset$.
The space of feasible solutions $\mathcal{X}^C$ is defined as 
\begin{align}
\nonumber 
y'_{uv} &\in \{0,1\}, y \in \{0,1\}^C: \quad y'_{uv} \leq \sum_{ij\in C}y_{ij}\,,\\
\nonumber &\forall i\in A: \sum_{ij\in C} y_{ij}\leq 1 \,,\quad \forall j\in B: \sum_{ij\in C} y_{ij}\leq 1\,, \\
 &uv\in C \Rightarrow y'_{uv}\geq y_{uv}\,.
\end{align}
The constraints stipulate that
(i)~the lifted edge $uv$ is $0$ if all the edges in the cut are $0$,
(ii)~there exists at most one active outgoing resp.\ incoming edge for every vertex in $A$ resp.\ $B$ and
(iii)~if there is also base edge $uv\in C$ then whenever it is active, the lifted  edge $uv$ must be active.

\begin{algorithm}
\caption{Cut-Subproblem-Optimization}
\label{alg:cut-subproblem-optimization}
 \textbf{Input} Edge costs $\theta^C$\\
 \textbf{Output} optimal value $\mathrm{opt}$ of subproblem.
    \begin{algorithmic}[1]
%\State    \Comment{Construct linear assignment problem}\\
\State Define $\psi \in \R^{{A} \times {B}}$:
\State $\psi_{ij} = \begin{cases}
    \theta^C_{uv} + \theta'^C_{uv},& \text{if }ij=uv\wedge uv\in C \wedge \theta'^C_{uv} > 0 \\
    \infty,& \text{if }ij \notin C\\
    \theta^C_{ij},& \text{otherwise} 
\end{cases}$
 %  \State $\forall ij\in C: \psi_{ij} = \theta^C_{ij} $
 %  \State $\forall ij\in A\times B\setminus C: \psi_{ij}=0$
 %  \IIf{$uv\in C\wedge \theta^C_{uv}>0$} $\psi^C_{uv}+=\theta'^C_{uv}$ 
    \State $z^* \in \argmin\limits_{z \in \{0,1\}^{{A}\times{B}}} \sum\limits_{i\in A}\sum\limits_{j\in B} \psi_{ij}z_{ij}$,\ s.t.\  $z \mathbbmss{1} \leq \mathbbmss{1}, z^\top \mathbbmss{1} \leq \mathbbmss{1}$
    \State $\mathrm{opt}=\sum_{ij\in C}\psi_{ij} z^*_{ij}$
    \IIf{$\theta'^C_{uv}\geq 0$} return $\mathrm{opt}$
   % \If{$\forall ij\in A\times B: z_{ij}=0$}
    \If{$\exists kl\in C: z_{kl}=1$}
    \State return $\mathrm{opt}+\theta'^C_{uv}$
   % \IIf{$\alpha< \theta^C_{uv}$} $opt=$
    \Else
        \State $\alpha =\min_{ij\in C}\theta^C_{ij}$
    \IIf{$ |\theta'^C_{uv}|> \alpha$} return $\theta'^C_{uv}+\alpha$
    \EElse return $\mathrm{opt}$ 
    \EndIf
    \end{algorithmic}
\end{algorithm}

\myparagraph{Optimization of a~cut subproblem}  with respect to feasible set $\mathcal{X}^C$ is given by Alg.~\ref{alg:cut-subproblem-optimization}. 
Its key is to solve a linear assignment problem (LAP) \cite{ahuja1988network} between vertex sets $A$ and $B$.
The assignment cost $\psi_{ij}$ for $(i,j)\in  A\times B$ is the cut edge cost $\theta^C_{ij}$ if edge $ij$ belongs to $C$ and $\infty$ otherwise. 
In the special case of $uv\mhyphen\text{cut }C$ containing base edge $uv$ and the lifted edge cost $\theta'^C_{uv}$ being positive, the assignment cost $\psi_{uv}$ is increased by $\theta'^C_{uv}$. 

A candidate optimal labeling of cut edges is given by values of LAP variables $z_{ij}$.
If $\theta'^C_{uv}\geq 0$, the optimal value found by the LAP is the optimal value of the cut subproblem.
If it is negative, we distinguish two cases: 
(i)~If a cut edge $kl$ labeled by one exists, the lifted edge cost $\theta'^C_{uv}$ is added to the optimal value of LAP.
(ii)~Otherwise, we inspect whether it is better to activate the smallest-cost cut edge and the lifted edge $uv$ or keep all edges inactive.

We use a~variation  of Alg.~\ref{alg:cut-subproblem-optimization} with an edge variable restricted to be either $0$ or $1$ for computing min-marginals.
%We obtain min marginals of the cut subproblem by modifying Alg,~\ref{alg:cut-subproblem-optimization} such that an edge variable is restricted to be zero or one.


\andrea{I changed the notation of node variables to $z$ because of confusion with $x$ in general subproblem. However, in Alg. \ref{alg:cut-subproblem-optimization} we have now confusion of $z$.}
% \begin{algorithm}
% \caption{Cut-Subproblem-Optimization}
% \label{alg:cut-subproblem-optimization}
%  \textbf{Input} Edge costs $\theta^C$\\
%  \textbf{Output} optimal value $opt$ of subproblem.
%     \begin{algorithmic}[1]
% %\State    \Comment{Construct linear assignment problem}\\
% \State Define $\psi \in \R^{{A} \times {B}}$:
% \State $\psi_{ij} = \begin{cases}
%     \theta^C_{uv} + \theta'^C_{uv},& uv \in C, \theta'^C_{uv} > 0 \\
%     \infty,& ij \notin C\\
%     \theta^C_{ij},& \text{otherwise} 
% \end{cases}$
%  %  \State $\forall ij\in C: \psi_{ij} = \theta^C_{ij} $
%  %  \State $\forall ij\in A\times B\setminus C: \psi_{ij}=0$
%  %  \IIf{$uv\in C\wedge \theta^C_{uv}>0$} $\psi^C_{uv}+=\theta'^C_{uv}$ 
%     \State $z^* \in \argmin\limits_{z \in \{0,1\}^{{A} \times {B}}} \la \psi, z\ra$\quad s.t.\ \quad $z \mathbbmss{1} \leq 1, z^\top \mathbbmss{1} \leq 1$
%     \State $\mathrm{opt}=\sum_{ij\in C}\psi_{ij} z^*_{ij}$
%     \IIf{$\theta'^C_{uv}\geq 0$} return $\mathrm{opt}$
%   % \If{$\forall ij\in A\times B: z_{ij}=0$}
%     \If{$\exists kl\in C: z_{kl}=1$}
%     \State return $\mathrm{opt}+\theta'^C_{uv}$
%   % \IIf{$\alpha< \theta^C_{uv}$} $opt=$
%     \Else
%         \State $\alpha =\min_{ij\in C}\theta^C_{ij}$
%     \IIf{$ |\theta'^C_{uv}|> \alpha$} return $\theta'^C_{uv}+\alpha$
%     \EElse return $\mathrm{opt}$ 
%     \EndIf
%     \end{algorithmic}
% \end{algorithm}

\myparagraph{Cutting plane.} There are exponentially many cut subproblems.
Therefore, we add only those that improve the lower bound.
See Appendix~\ref{sec:cutting-planes-cut-subproblems} for details.

% \myparagraph{Cutting plane.} Similarly as for the path subproblems, there are exponentially many cut subproblems.
% Therefore, we add only those that improve the lower bound.
% See Section~\ref{sec:cutting-planes-cut-subproblems} in the Appendix for details.

\subsection{Message Passing}

The overall algorithm for optimizing the Lagrange decomposition is Alg.~\ref{alg:message-passing} in the Appendix.
First, inflow and outflow subproblems are initialized for every node.
%of the original graph $G=(V,E)$.
Then, for a number of iterations or until convergence, costs for each subproblems are adjusted iteratively by computing min-marginals and adjusting the reparametrization  proportionally to the min-marginal's value.
Additionally, every $k$-th iteration additional path and cut subproblems are separated and added to the Lagrange decomposition.  

\myparagraph{Solver complexity.} 
We need $\mathcal{O}(|E^{inp}|)$ space where $E^{inp}$ are all edges before graph sparsification. 
% A detailed time complexity analysis per algorithm is provided in Appendix~7.13.
%We provide detailed time complexity analysis in Appendix~\ref{appendix:runtime} analyses time complexity.
The most time consuming is computing lifted edges min-marginals  for each in/outflow subproblem. Alg.~\ref{ap:alg:all-lifted-mm} computes them for one outflow subproblem and it is linear in the number of detections per frame. 
% Overall, the most time consuming procedure of the solver is Algorithm 6 with a quadratic runtime in the number of detections in a frame. 
This significantly improves the complexity of to the optimal LDP solver LifT, making LDP applicable to large problem instances. 
See Appendix~\ref{appendix:runtime} for details.
%Details in Appendix~\ref{appendix:runtime}.

% \myparagraph{Solver complexity.} 
% We need $\mathcal{O}(|E^{inp}|)$ space where $E^{inp}$ are edges provided to the solver before graph sparsification. 
% We provide detailed time complexity analysis in Appendix~\ref{appendix:runtime}.
% The most time consuming procedure is calling Alg.~\ref{ap:alg:all-lifted-mm} 
% %(min-marginals of lifted edges in in/outflow subproblems)
% for each vertex where Alg.~\ref{ap:alg:all-lifted-mm} is linear in the number of detections per frame. 
% % Overall, the most time consuming procedure of the solver is Algorithm 6 with a quadratic runtime in the number of detections in a frame. 
% This significantly improves the time complexity bound compared to the optimal LDP solver LifT, making LDP applicable to large problem instances. 

\subsection{Primal Rounding}\label{sec:primal-rounding}
For computing primal solutions we solve a minimum cost flow (MCF) problem on the base edges and improve this initial solution with a local search heuristic.

Without lifted edges, the disjoint paths problem is an instance of MCF, which can be efficiently optimized via combinatorial solvers like the successive shortest path solver that we employ~\cite{ahuja1988network}.
We enforce node disjoint paths via splitting each node $u\in V$ into two nodes $u^{in},u^{out}\in V^{mcf}$ in the MCF graph $G^{mcf}=(V^{mcf},E^{mcf})$, adding an additional edge $u^{in}u^{out}$ to $E^{mcf}$ and setting capacity $[0,1]$ on all edges $E^{mcf}$. 
%This ensures at most one incoming resp.\ outgoing edge via flow conservation.
%All edges in $E^{mcf}$ are directed and have capacities in $[0,1]$.
Each node except $s$ and $t$ has demand $0$.
%  Alg.~\ref{alg:mcf-init} details how edge costs for the MCF  are calculated from the edge costs of inflow and outflow subproblems via calling Alg.~\ref{alg:outflow-minimization}.
% We obtain the cost of each flow edge $u^{out}v^{in}$
% from the inflow subproblem of $v$ and the outflow subproblem of $u$ using their minima where edge $uv$ is active.
Alg.~\ref{alg:mcf-init} calculates MCF edge costs from in/outflow subproblems using Alg.~\ref{alg:outflow-minimization}.
We obtain the cost of each flow edge $u^{out}v^{in}$
from the inflow subproblem of $v$ and the outflow subproblem of $u$ using their minima where edge $uv$ is active. This combines well the cost from base and lifted edges. 

%contains the best cost achievable by activating $uv$ in the outflow  subproblem of $u$ plus the best cost achievable by activation $uv$ in the inflow subproblem of $v$.
%So that cost of each edge $vw\in E$ is synthesized from costs of all lifted edges adjacent to $v$ and $w$. 

We describe the local search heuristic for improving the MCF solution in Alg.~\ref{alg:post-process-primal} in the Appendix.
% The local search heuristic for improving the MCF solution is described in Algorithm~\ref{alg:post-process-primal} in the Appendix.
It works with sets of disjoint paths.
First, paths are split if this leads to a decrease in the objective.
%
Second, merges are explored.
If a merge of two paths is not possible, we iteratively check whether cutting off one node from the first path's end or the second paths's beginning makes the connection possible.
If yes and the connection is decreasing the objective, the nodes are cut off and the paths are connected.

\begin{algorithm}
\caption{Init-MCF}
\label{alg:mcf-init}
    \begin{algorithmic}[1]
    \State  \begin{varwidth}[t]{\linewidth}
    $\forall u \in V\backslash \{s,t\}$: \par
     $(o,lc,\alpha^{in})$=Opt-In-Cost$(u,\theta^{in}_u)$\par
     $(o,lc,\alpha^{out})$=Opt-Out-Cost$(u,\theta^{out}_u)$
    \end{varwidth}
    \State $\forall u \in V\backslash \{s,t\}:$ $\theta^{mcf}_{s u^{in}} = \alpha^{in}_{su}$, $\theta^{mcf}_{u^{out} t} = \alpha^{out}_{ut}$
    \State 
    \begin{varwidth}[t]{\linewidth}
    $\forall u \in \{uv \in E| u \neq s, v \neq t\}:$
    $\theta^{mcf}_{u^{out} v^{in}} = \alpha^{out}_{uv} + \alpha^{in}_{uv}$
    \end{varwidth}
    \end{algorithmic}
\end{algorithm} 



==> lifted disjoint paths message passing/ablationTable.tex <==
\begin{center}
\begin{table}
\setlength{\tabcolsep}{3pt}
\def\arraystretch{0.8}
%\caption{Ablations on MOT17 train without postprocessing.
\caption{Influence of lifted graph sparsification, message passing and using zero base costs on MOT17 train without postprocessing.%Message passing is disabled for \textit{w/o MP}, for (i) w/o Base edge costs set to zero (3) w/o Base edge costs set to zero and sparser lifted graph (4) w/o message passing}
}
\label{tab:ablations}
\small{
\begin{tabularx}{\columnwidth}{cccccccc}
\toprule
 \multirow{2}{*}{$E'$} & MP & Base & \multirow{2}{*}{IDF1$\uparrow$}&  \multirow{2}{*}{MOTA$\uparrow$}
& \multirow{2}{*}{FP$\downarrow$}& \multirow{2}{*}{FN$\downarrow$}&  \multirow{2}{*}{IDS$\downarrow$} \\
&steps & cost & & & & & \\
\midrule
Dense        & $82$ & Zero      & $\mathbf{71.0}$ & $\mathbf{66.3}$& $2826$  & $\mathbf{109263}$ & $1369$ \\
Dense        & $0$  & Zero      & $70.3$ & $\mathbf{66.3}$ & $2832$  & $109265$ & $1354$        \\
Dense        & $82$ & Orig.     & $69.8$ &$\mathbf{66.3}$& $\mathbf{2824}$  & $109266$ & $1355$    \\
Sparse       & $82$ & Orig.     & $69.1$ & $\mathbf{66.3}$ & $2825$  & $\mathbf{109263}$ & $\mathbf{1316}$     \\
\bottomrule
\end{tabularx}
}
\vspace{-2.5mm}
\end{table}
%\vspace*{-25mm}

\end{center}

==> lifted disjoint paths message passing/abstract.tex <==
\begin{abstract}
 We present an efficient approximate message passing solver for the lifted disjoint paths problem (LDP), a natural but NP-hard model for multiple object tracking (MOT).
 Our tracker scales to very large instances that come from long and crowded MOT sequences.
 Our approximate solver enables us to process the MOT15/16/17 benchmarks  without sacrificing solution quality and allows for solving MOT20, which has been out of reach up to now for LDP solvers due to its size and complexity.
  On all these four standard MOT benchmarks we achieve performance comparable or better than  current state-of-the-art methods including a tracker based on an optimal LDP solver.
%%Previous version
% We present an efficient message passing solver for the lifted disjoint paths problem (LDP), a natural model for multiple object tracking.
% Our solver scales to very large instances that come from long and crowded multiple object tracking problem sequences.
% Our solver enables us to solve the MOT17 benchmark without sacrificing solution quality and allows for solving MOT20, which has been out of reach up to now for LDP-solvers.
%  We achieve the performance of previous LDP solvers on MOT17 and performance comparable to state-of-the-art trackers on MOT20.



%%CMT version:
% We present an efficient message passing solver for the lifted disjoint paths problem (LDP), a natural model for multiple object tracking. In contrast to previous solvers for LDP, our solver is more efficient and scales to large multiple object tracking problems that come from long and crowded sequences. Our solver enables us to solve the MOT17 benchmark without sacrificing solution quality and allows for solving MOT20, which has been out of reach up to now for LDP-solvers. We achieve the performance of previous LDP solvers on MOT17 and performance comparable to state-of-the-art trackers on MOT20.



% We present an efficient message passing solver for the lifted disjoint paths problem (LDP), a natural model for multiple object tracking.
% Our solver scales to very large instances that come from long and crowded multiple object tracking problem sequences.
% %In contrast to previous solvers for LDP, our solver is more efficient and scales to large multiple object tracking problems that come from long and crowded sequences.
% %Our solver enables us to solve the MOT17 benchmark significantly faster without sacrificing solution quality and allows for solving MOT20, which has been out of reach up to now for LDP-solvers.
% Our solver enables us to solve the MOT17 benchmark without sacrificing solution quality and allows for solving MOT20, which has been out of reach up to now for LDP-solvers.
% %We achieve the performance of previous LDP solvers on MOT17 and obtain state-of-the-art results on MOT20.
%  We achieve the performance of previous LDP solvers on MOT17 and performance comparable to state-of-the-art trackers on MOT20.
\end{abstract}


==> lifted disjoint paths message passing/acknowledgements.tex <==
\section{Acknowledgements}
This work was supported by the Federal Ministry of Education and Research (BMBF), Germany, under the project LeibnizKILabor (grant no.\ 01DD20003), the Center for Digital Innovations
(ZDIN) and the Deutsche Forschungsgemeinschaft (DFG) under Germany’s Excellence Strategy
within the Cluster of Excellence PhoenixD (EXC 2122).

% This work has been supported by the Federal Ministry of Education and Research (BMBF), Germany, under the project LeibnizKILabor (grant no. 01DD20003), the Center for Digital Innovations
% (ZDIN) and the Deutsche Forschungsgemeinschaft (DFG) under Germany’s Excellence Strategy
% within the Cluster of Excellence PhoenixD (EXC 2122).

==> lifted disjoint paths message passing/bigTable.tex <==

\begin{table*}
\center
\def\arraystretch{0.9}%  1 is the default, change whatever you need
\small{
%\tabcolsep=0.09cm
    \caption{Comparison of ApLift with the best performing solvers w.r.t.\ MOTA metric on the MOT challenge. $\uparrow$ higher is better,  $\downarrow$ lower is better. The two rightmost columns: average number of frames per sequence and the average number of detections per frame for dataset.} 


    \begin{tabular}{c c  c c c c c c c c c c }
    
    
     \toprule
     & Method  & MOTA$\uparrow$  & IDF1$\uparrow$  & MT$\uparrow$  & ML$\downarrow$  & FP$\downarrow$ & FN$\downarrow$ & IDS$\downarrow$ & Frag$\downarrow$ & Frames & Density \\   
     \toprule
     
     \parbox[t]{3mm}{\multirow{3}{*}{\rotatebox[origin=c]{90}{MOT20}}} 
& ApLift (ours) & $\mathbf{58.9}$ & $56.5$ & $\mathbf{513}$ & $\mathbf{264}$ & $17739$ & $\mathbf{192736}$ & $2241$ & $2112$ & \multirow{3}{*}{1119.8} & \multirow{3}{*}{170.9} \\ % frames 4479
& MPNTrack~\cite{braso2020learning} & $57.6$ & $\mathbf{59.1}$ & $474$ & $279$ & $16953$ & $201384$ & $\mathbf{1210}$ & $\mathbf{1420}$ & & \\ 
& Tracktor++v2~\cite{bergmann2019tracking} & $52.6$ & $52.7$ & $365$ & $331$ & $\mathbf{6930}$ & $236680$ & $1648$ & $4374$ & & \\ 
     \midrule

     \parbox[t]{3mm}{\multirow{4}{*}{\rotatebox[origin=c]{90}{MOT17}}} 
& CTTrackPub~\cite{zhou2021tracking} &  $\mathbf{61.5}$ & $59.6$ & $621$ & $752 $ & $\mathbf{14076}$ & $200672$ & $2583$ & $4965$ & \multirow{4}{*}{845.6} &\multirow{4}{*}{31.8} \\ % frames 17757
& ApLift (ours) & $60.5$ & $\mathbf{65.6}$ & $\mathbf{798}$ & $\mathbf{728}$ & $30609$ & $\mathbf{190670}$ & $1709$ & $2672$ & & \\ 
& Lif\_T~\cite{hornakova2020lifted} &  $60.5$ &$ \mathbf{65.6} $& $637 $ & $791$  & $14966$ & $206619$ & $1189 $& $3476$ & & \\ 
& MPNTrack~\cite{braso2020learning} & $58.8$ & $61.7$ & $679$ & $788$ & $17416$ & $213594$ & $\mathbf{1185}$ & $\mathbf{2265}$ & &  \\

     \midrule
     
     \parbox[t]{3mm}{\multirow{4}{*}{\rotatebox[origin=c]{90}{MOT16}}} 
&ApLift (ours) & $\mathbf{61.7}$ & $\mathbf{66.1}$ & $\mathbf{260}$ & $\mathbf{237}$ & $9168$ & $\mathbf{60180}$ & $495$ & $802$ & \multirow{4}{*}{845.6} & \multirow{4}{*}{30.8}\\ % 5919 frames
&Lif\_T~\cite{hornakova2020lifted}  &  $61.3 $& $64.7$ & $205$ & $258$ & $4844$ & $65401$ & $389$ & $1034$ & & \\ 
& MPNTrack~\cite{braso2020learning} & $58.6$ & $61.7$ & $207$ & $258$ & $4949$ & $70252$ & $\mathbf{354}$ & $\mathbf{684}$ & & \\ 
& GSM~\cite{ijcai2020-74} & $57.0$ & $55.0$ & $167$ & $262$ & $\mathbf{4332}$ & $73573$ & $475$ & $859$ & & \\ 

     \midrule
     
     \parbox[t]{3mm}{\multirow{4}{*}{\rotatebox[origin=c]{90}{MOT15}}} 
& Lif\_T~\cite{hornakova2020lifted}  &  $\mathbf{52.5}$ & $\mathbf{60.0}$ & $244 $ & $186$ & $6837$ & $21610$ & $730$ & $1047$ & \multirow{4}{*}{525.7} & \multirow{4}{*}{10.8} \\ % 5783 frames
& MPNTrack~\cite{braso2020learning} & $ 51.5 $& $58.6$ & $225$ & $187$ & $7260$ & $21780$ & $\mathbf{375}$ & $\mathbf{872}$ & &  \\ 
& ApLift (ours) & $51.1$ & $59.0$ & $\mathbf{284}$ & $\mathbf{163}$ & $10070$ & $\mathbf{19288}$ & $677$ & $1022$ & & \\ 
& Tracktor15~\cite{bergmann2019tracking} & $ 44.1 $& $46.7$ & $130$ & $189$ & $\mathbf{6477}$ & $26577$ & $1318$ & $1790$ & &  \\ 

     \bottomrule
    \end{tabular}


\label{tab:mot}
}
\vspace{-5mm}
\end{table*}


==> lifted disjoint paths message passing/conclusion.tex <==
\section{Conclusion}
%We made the NP-hard LDP concept applicable for processing massive sequences of MOT20 by the combination of an approximate solver, efficient input costs and subdivision of data keeping sufficient context for each decision.
We demonstrated that the NP-hard LDP model is applicable  for processing massive sequences of MOT20. The combination of an approximate LDP solver, efficiently computable costs and subdivision of data keeping sufficient context for each decision make this possible.
 %We proved that the NP-hard LDP concept can be used for processing massive sequences of MOT20. The combination of an approximate LDP solver, input costs based on effective features and subdivision of data providing sufficiently broad context for each  decision make this possible.


% I

% want

% too 

% see

% how

% much 

% space 

% we

% have

% to

% write

% the

% conclusion

==> lifted disjoint paths message passing/experiments.tex <==
\section{Experiments}
\label{sec:experiments}
We integrate our LDP solver into an MOT system (Appendix, Fig. \ref{fig:overallframework}) and show
%demonstrate 
on 
%several 
challenging datasets that higher order MOT is scalable to big problem instances.
%Additional evaluations are provided in Appendix, 
In the next sections, we describe our experimental setup and present results. We clarify the edge cost calculation and construction of the base and the lifted graph and their sparsification. %The tracking system is shown in Figure \ref{fig:overallframework}. 


\subsection{Pairwise Costs}
\label{sec:cost_classifier}
We use multi layer perceptrons (MLP) to predict the likelihood that two detections belong to the same trajectory.
We divide the maximal frame distance into $20$ intervals of equal length and train one separate MLP for each set of frame distances.
 We transform the MLP output to the cost of the edge between the detections and use it in our objective~\eqref{eq:lifted-disjoint-paths-problem}.
Negative cost indicates that two detections belong to the same trajectory. Positive cost reflects the opposite.

%\noindent{\textbf{MLP architecture:}} 
\myparagraph{MLP architecture.}
Each MLP consists of a fully connected layer with the same number of neurons as the input size, followed by a LeakyReLU activation \cite{maasrectifier} and a~fully connected single neuron output layer. We add sigmoid activation in the training. 
We describe our spatial and visual features used as the input in the paragraphs below.

%\noindent{\textbf{Spatial Feature:}}
\myparagraph{Spatial feature} uses bounding box information of two detections $v$ and $w$. We align the boxes such that their centers overlap. The similarity feature $\sigma_{vw,\text{Spa}} \in [0, 1]$ is the intersection-over-union between two aligned boxes.

\myparagraph{Appearance feature.}
%\label{section:visual_feature}
We create an appearance feature $F_{v}$ for each detection $v$  by training the method  \cite{zheng2019joint}  on the training set of the respective benchmark and additional data from \cite{zheng2015scalable, wei2018person, ristani2016MTMC}. The similarity feature $\sigma_{vw,\text{App}}$ between detection $v$ and $w$ given by \mbox{$\sigma_{vw,\text{App}}:=\max\{0,\la F_v, F_{w}\ra\}$} is used. A higher value indicates a higher similarity. 

\myparagraph{Global context normalization.}
The two features $\sigma_{vw,\text{Spa}}$, $\sigma_{vw,\text{App}}$ depend entirely on the nodes $v$ and $w$. 
To include global context, we append several normalized versions of the two features to the edge feature vector, inspired by \cite{hornakova2020lifted}.
Both features $\sigma_{ij,*}$ of edge $ij$ undergo a~five-way normalization. 
In each case, the maximum feature value from a~relevant set of edges is selected as the normalization value.
The normalization is done by dividing the two features $\sigma_{ij,*}$ by each of their five normalization values. This yields 10 values.
Another set of 10 values for edge $ij$ is obtained by dividing $\sigma^2_{ij,*}$ by each of the five normalization values.
Together with the two unnormalized features $\sigma_{ij,*}$, edge feature vectors have length 22.
See Appendix~\ref{appendix:feature_scaling} for details.

\myparagraph{Training.} 
We iteratively train our MLP on batches $B$ containing sampled edges. To compensate the imbalance between true positive and true negative edges, we use an $\alpha$-balanced focal loss \cite{focalLoss} with $\gamma=1$. We define the $\alpha$-weight $\alpha^{(g,\Delta f)}$ to weight the correct classification of edge $vw$ with ground truth flow value $g_{vw} \in \{0,1\}$, time distance $\Delta f$ between $v$  in frame $f_{v}$ and $w$ in frame $f_{w}$, and value $g \in \{0,1\}$ via {$\alpha^{(g,\Delta f)} := 1/| \{vw \in E: |f_{v} -f_{w}| = \Delta f, g_{vw} = g \} |\, .$}
We optimize the classifier using Adam with $l_r=0.1$, $\beta_1=0.9$, $\beta_2=0.999$ and $\epsilon=10^{-8}$. 
To reduce complexity while maintaining  variety during training, we introduce an extended sampling. Given a frame $f$, we create batches $B(f)$ by sampling detections from a fixed sequence of frame shifts starting at frame $f$ ensuring that all temporal distances $\Delta f$ are present in $B(f)$ (details in Appendix \ref{appendix:sampling}). We then subsample the $k$-nearest detections to a random generated image position with $k=160$, which sensitizes  training to crowded scenes. We train the MLP for $3$ epochs with batches $B(f)$ for all frames $f$ of the dataset.



\subsection{Graph Construction}
\label{sec:graph_construction}
We create the base and the lifted graph edges between detections with time distance up to $2$ seconds.
% We create the base and the lifted graph with edges between detections within time distance up to $2$ seconds.
We also add an edge from source $s$, and to sink $t$ to each detection.
In order to reduce computational complexity, we apply sparsification on both base and lifted graph as described later. 
\andrea{I would move first sentence of the Cost paragraph to graph sparsification. The rest of the paragraph should go to Section Cost Classifier which would be renamed to "Cost" or something.}

\myparagraph{Costs.}
%For each edge $vw\in E \cup E'$, negative edge cost indicates that two detections belong to the same trajectory, while positive cost reflect the opposite. 
We obtain base and lifted costs $c$ and $c'$ from the same MLP classifier (Sec.~\ref{sec:cost_classifier}). 
%
Due to decreasing classification accuracy with increasing frame distance $\Delta f$, we multiply the costs by a decay weight $\omega_{\Delta f} \coloneqq (10 \cdot \Delta f + 0.1)^{-1}$, so that edges representing long temporal distances have lower weight.
Edges from $s$ and  to $t$ have costs zero. 
% Outgoing edges from $s$ and incoming edges to $t$ have their costs fixed to zero. 


Finally, we use simple heuristics to find pairs that are obviously matching or non-matching.
We set the corresponding costs to be high in absolute value, negative for matching and positive for non-matching, thereby inducing soft constrains. 
An obvious match is given by a nearly maximal feature similarity. Detection pairs are obviously non-matching, if the displacement between their bounding boxes is too high.
%Obviously disconnected detections are determined by implausible high displacements between detection boxes.
See  Appendix~\ref{appendix:high_confident} for details.
% Finally, we use simple heuristics to find pairs that should be obviously connected or obviously disconnected. We set the corresponding costs to be high in absolute value. These costs are negative for obvious joints and positive for obvious cuts, thereby inducing soft-constrains. Edges are obviously connected, if the corresponding feature similarity is nearly optimal. Detections are obviously disconnected, if the displacement between their bouning boxes is too high.
% %Obviously disconnected detections are determined by implausible high displacements between detection boxes.
% See Sec. \ref{appendix:high_confident} in the Appendix for details.


\myparagraph{Sparsification.}
%\myparagraph{Sparsification.}
The base edges are an intersection of two edge sets. The first set contains for every $v \in V'$ edges to its $3$ nearest (lowest-cost) neighbors from every subsequent time frame. 
%The second set contains for every $v \in V'$ edges to its $3$ nearest neighbors from every preceding  frame. 
The second set selects for every vertex the best edges to its preceding frames analogically.
%Edges longer than 6 frames  must additionally comply with maximal cost threshold $3.0$.
Moreover, edges longer than 6 frames  must have costs lower than $3.0$.
To avoid double counting of edge costs, we subsequently set costs of all base edges between non-consecutive frames to zero, so that only  lifted edges maintain the costs. 
If a~lifted edge has cost around zero, it is not discriminative and we remove it, unless it overlaps with a~(zero-valued) base edge. 
% For lifted graph, edges having cost around zero  are not discriminative. We remove such edge unless it overlaps with a~(zero-valued) base edge. 



\input{bigTable}

%\vspace{-18.2mm}
\subsection{Inference}
For fair comparison to state of the art, we filter and refine detections using tracktor~\cite{bergmann2019tracking} as in \cite{hornakova2020lifted}. Different to \cite{hornakova2020lifted}, we apply tracktor to recover missing detections before running the solver.
% Before we apply our method, we follow \cite{hornakova2020lifted,braso2020learning} and use tracktor \cite{bergmann2019tracking} to filter and refine input detections. Different to \cite{hornakova2020lifted}, we apply the recovery before running the solver.

While we solve MOT15/16/17 on global graphs,  we solve MOT20 in time intervals in order to decrease memory consumption and runtime.
First, we solve the problem on non-overlapping adjacent intervals and fix the trajectories in the interval centers. Second, we solve the problem on a new set of intervals where each of them covers unassigned detections in two initial neighboring intervals and enables connections to the fixed trajectory fragments.
We use the maximal edge length of 50 frames in MOT20. Therefore, 150 is the minimal interval length such that all edges from a~detection are used when assigning the detection to a~trajectory. This way, the solver has sufficient context for making each decision.
Intervals longer than 200 frames increase the complexity significantly for MOT20, therefore we use interval length 150 in our experiments.


 % Details in Section \ref{sec:intervalSolution} in the Appendix. 


\myparagraph{Post-processing.} We use simple heuristics to check if base edges over long time gaps correspond to plausible motions, and split trajectories if necessary.
Finally, we use linear interpolation to recover missing detections within a trajectory. 
%See details in Appendix \ref{appendix:post_processing}).  
%Further details on inference can be found in the
Appendix~\ref{sec:inference} contains further details on inference.



% \myparagraph{Solver complexity} 
% We need $\mathcal{O}(|E^{inp}|)$ space where $E^{inp}$ are edges provided to the solver before graph sparsification. 
% % A detailed time complexity analysis per algorithm is provided in Appendix~7.13.
% We provide detailed time complexity analysis in Appendix~\ref{appendix:runtime}.
% The most time consuming procedure is calling Alg.~\ref{ap:alg:all-lifted-mm} for each vertex where Alg.~\ref{ap:alg:all-lifted-mm} is linear in the number of detections per frame. 
% % Overall, the most time consuming procedure of the solver is Algorithm 6 with a quadratic runtime in the number of detections in a frame. 
% This significantly improves the time complexity bound compared to the optimal LDP solver LifT, making LDP applicable to large problem instances. 
%To demonstrate this, we compare 
% We compare
% the runtime of our solver against  two step procedure of LifT for a~sample sequence in Table \ref{tabel:runtime}. 
% With increasing problem complexity, our solver outperforms LifT w.r.t.\ runtime while achieving similar results w.r.t. tracking metrics. Note that better objective value in terms of LDP~\eqref{eq:lifted-disjoint-paths-problem} does not automatically translate to better MOT metrics due to imperfect input costs. Therefore, we may sometimes observe slightly worse IDF1 score for better LDP solutions.  We provide comparison of our solver against optimal (one step) LifT on MOT17 train in Appendix~\ref{appendix:runtime}. 

\subsection{Tracking Evaluation}
 
We evaluate our method on four standard MOT benchmarks.
The MOT15/16/17 benchmarks \cite{MOTChallenge2015,MOT16} contain semi-crowded videos sequences filmed from a~static or a~moving camera. 
MOT20 \cite{MOTChallenge20} comprises crowded scenes with considerably higher number of  frames  and detections per frame, see Tab.~\ref{tab:mot}.
% MOT20 \cite{MOTChallenge20} comprises crowded scenes with an average number of  frames and average number of detections per frame considerably higher than for MOT15/16/17. 
% Note that the number of edges in our graphs grows quadratically with the number of detections per frame. Therefore,  it was crucial to make the tracker scalable to these massive data. 
The challenge does not come only with the data size. Detectors make more errors in crowded scenes due to frequent occlusions and appearance features are less discriminative as the distance of people to the camera is high. 
Using higher order information helps in this context. However, the number of edges in our graphs grows quadratically with the number of detections per frame. Therefore, it is crucial to make the tracker scalable to these massive data. 
We use the following ingredients to solve the problems: (i)~fast but accurate method for obtaining edge costs, (ii)~approximate LDP solver delivering high-quality results fast, (iii)~preprocessing heuristics, (iv)~interval solution keeping sufficient context for each decision. 

We use training data of the corresponding dataset for training and the public detections for training and test. 
\vspace{-6mm}
\input{ablationTable}
\vspace{-8mm}
\input{runtimeTableMOT20-1}
\vspace{-10mm}

% We trained our method based on the training data of the corresponding dataset, and use the public detections for training and test. 

We compare our method using standard MOT metrics. MOTA \cite{motametric} and IDF1 \cite{IDF1metric} are considered  the most representative  as they incorporate other metrics (in particular recall and precision).
% We compare our method using the most representative standard MOT metrics MOTA \cite{motametric} and IDF1 \cite{IDF1metric}.
%Thereby, 
IDF1 is more penalized by inconsistent trajectories. We also report mostly tracked (MT) and mostly lost trajectories (ML), false negatives (FN) and false  positives (FP), ID switches (IDS) and fragmentations (Frag) as provided by the evaluation protocols \cite{motametric} of the benchmarks.

% The comparison to top peer-reviewed methods on test sets is shown in Table \ref{tab:mot}.



Tab.~\ref{tab:mot} shows the comparison to the best (w.r.t.\ MOTA)  peer-reviewed methods  on test sets.
Our approximate solver achieves almost the same results on  MOT15/16/17 as the optimal LDP solver~\cite{hornakova2020lifted}, while using simpler features.
%
% MOTA and IDF1 are considered the most relevant metrics in MOT as they incorporate other metrics (in particular recall and precision). Here, ApLift performs comparable or better than current state-of-the-art methods.
% Overall, our method performs on par with state-of-the-art on all evaluated benchmarks. 
%
Overall, our method performs on par with state  of the art on all evaluated benchmarks, especially in MOTA and IDF1. %that are considered the most relevant MOT metics.
Our complete results and videos are publicly available\footnote{\scriptsize \url{https://motchallenge.net/method/MOT=4031&chl=13}}.
% We trained our method based on the training data of the corresponding dataset, and use the public detections for training and test. 
%
The proposed method achieves overall low FN values but slightly high FP values. 
%It is hard to identify a~tracker component that influences a~specific metric.
%In our case, 
FP/FN are mostly affected by preprocessing the input detections and interpolation in the post-processing. The impact of post-processing (trajectory splits and interpolations) on MOT20, which causes FP but reduces FN and IDS, is analyzed in the Appendix (Tab.~\ref{tab:postprocessing}).  
% MOTA and IDF1 are considered the most relevant metrics in MOT as they incorporate other metrics (in particular recall and precision). Here, ApLift performs comparable or better than current state-of-the-art methods.

Tab.~\ref{tab:ablations} shows the influence of various settings on the performance of MOT17 train.
%In particular, using dense or sparsified lifted graph, using message passing and setting the base cost to zero (see Sec.~5.1) or keep the original values. 82 MP iterations to correspond to the setup from Tab.~\ref{tab:mot}.
While we usually set the base edge costs to zero (Sec.~\ref{sec:graph_construction}), we need to keep them when using the sparsified lifted graph.
% Note that we need to keep the base edge costs when using the sparsified lifted graph.
% While we set it to zero usually (Sec.~\ref{sec:graph_construction}).
%Sec.~\ref{sec:graph_construction} explains how base edge costs are set to zero otherwise.
Both, message passing and dense lifted edges improve IDF1 and IDS. However, MOTA, FN and FP remain almost unchanged.


Finally, we compare
the runtime of our solver against the two step version of LifT for a~sample sequence in Tab.~\ref{tabel:runtime}.  
With increasing problem complexity, our solver outperforms LifT w.r.t.\ runtime while achieving similar IDF1. 
Counter-intuitively, as we progress towards increasingly better optimization objective values, the tracking metrics can slightly decrease due to imperfect edge costs.
We compare our solver against optimal (one step) LifT on MOT17 train in Appendix~\ref{appendix:runtime}. 

%Note that better LDP objective value~\eqref{eq:lifted-disjoint-paths-problem} does not automatically lead to better MOT metrics due to imperfect input costs. Therefore, we may sometimes observe slightly worse IDF1 for better LDP solutions.  











==> lifted disjoint paths message passing/formulation.tex <==
\section{Problem Formulation}
\label{sec:problem_formulation}
The lifted disjoint paths problem (LDP) introduced in~\cite{hornakova2020lifted} is an optimization problem for finding a set of vertex-disjoint paths in a~directed acyclic graph.
The cost of each path is determined by the cost of edges in that path as in the basic disjoint paths problem (DP), but additionally there are higher order costs defined by lifted edges.
A~lifted edge contributes to the cost if its endpoints are part of the same path.
%Through this, connectivity costs are incorporated in the basic disjoint paths problem.
This problem is a natural formulation for multiple object tracking (MOT), where lifted edges allow to re-identify the same objects over long distance.
%An example LDP is shown in Figure~\ref{fig:problemIllustration}.

While of greater expressivity, the LDP is NP-hard~\cite{hornakova2020lifted} in contrast to DP which is reducible to the minimum cost flow.
Below, we recapitulate the  formulation of LDP from~\cite{hornakova2020lifted}.


\subsection{Notation and Definitions.}
\begin{description} 
%\setlength{\parskip}{2pt}
 % \setlength\itemsep{0pt}
    \item[Flow network:] a directed acyclic graph $G = (V,E)$.
    \item[Start and terminal:] nodes $s,t \in V$.
    \item[Lifted graph:] a directed acyclic graph $G' = (V',E')$, where $V' = V \backslash\{s,t\}$.
%
    \item[The set of paths]
 starting at $v$ and ending in $w$ is
\begin{equation}
    vw\mhyphen\text{paths}(G) = \left\{ (v_1 v_2,\ldots,v_{l-1} v_l) : \begin{array}{c}v_i v_{i+1} \in E,\\ v_1 = v, v_l = w \end{array} \right\}\,.
\end{equation}
For a $vw\mhyphen$path $P$ its edge set is $P_E$ and its node set is $P_V$.

    \item[Reachability relation] for two nodes $v,w \in V$ is defined as $vw \in \mathcal{R}_G\Leftrightarrow vw\mhyphen\text{paths}(G) \neq \emptyset$.
    We assume that it is reflexive and $su \in \mathcal{R}_G, ut \in \mathcal{R}_G$  $\forall u \in V$, i.e.\ all nodes can be reached from  $s$ and all nodes can reach the sink node $t$.%
    % \item[Reachability relation] for two nodes $v,w \in V$ is defined as $vw \in \mathcal{R}_G\Leftrightarrow vw\mhyphen\text{paths}(G) \neq \emptyset$.
    % We assume that $su \in \mathcal{R}_G, ut \in \mathcal{R}_G$  $\forall u \in V$, i.e.\ all nodes can be reached from the source node $s$ and all nodes can reach the sink node $t$.
%
    \item[Flow variables:]
Variables $y \in \{0,1\}^E$ have value $1$ if flow passes through the respective edges.
%     \item[Node variables:]
% Node variables $z \in \{0,1\}^V$ denote flow passing through each node.
    \item[Node variables] $z \in \{0,1\}^V$ denote flow passing through each node. Values 0/1   forces paths to be node-disjoint.
    \item[Variables of the lifted edges] $E'$ are denoted by $y'\in\{0,1\}^{E'}$.
$y'_{vw}=1$ signifies that nodes $v$ and $w$ are connected via the flow $y$ in $G$.
%
Formally, 
\begin{equation}
\label{eq:lifted-edge-def}
y'_{vw} = 1 \Leftrightarrow \exists P\in vw\mhyphen\text{paths}(G): \forall ij\in P_E: y_{ij}=1 \,.
\end{equation}
\end{description}


\myparagraph{Lifted disjoint paths problem.}
Given edge costs $c \in \R^E$, node cost $d \in \R^V$ in flow network $G$ and edge cost $c' \in \R^{E'}$ for the lifted graph $G'$ the lifted disjoint paths problem is
\begin{equation}
\label{eq:lifted-disjoint-paths-problem}
\begin{array}{rl}
    \min\limits_{\substack{y \in \{0,1\}^E, y' \in \{0,1\}^{E'},\\ z \in \{0,1\}^{V}}} & \la c, y \ra + \la c',y' \ra + \la d, z\ra \\
    \text{s.t.} & y \text{ node-disjoint } s,t \text{-flow in } G, \\
                &z \text{ flow through nodes of }G\\
                & y, y' \text{ feasible according to } \eqref{eq:lifted-edge-def}
    \end{array}
\end{equation}

% Set $E'$ can be arbitrary.  Due to Formula~\eqref{eq:lifted-edge-def}, it makes sense to create a lifted edge $vw$ only if $vw\in \mathcal{R}_G$. Also, note that lifted edges between consecutive frames are not useful. We describe our choice in Sec.~\ref{sec:graph_construction}. 

Set $E'$ can be arbitrary.  It makes sense to create a~lifted edge $vw$ only if $vw\in \mathcal{R}_G$ due to Formula~\eqref{eq:lifted-edge-def} and only if $v$ and $w$ do not belong to neighboring frames. We describe our choice in Sec.~\ref{sec:graph_construction}. 

Other notation and abbreviations are in Appendix~\ref{ap:notation}.

% \begin{figure}
%     \centering
%     \includegraphics[width=0.4\textwidth]{illustrationNewNoT.pdf}
%     \caption{
%     Exemplary LDP: Black edges form the flow network $G$, \textcolor{blue}{blue} edges the lifted graph $G'$.
%     Bold edges have value $1$, while dashed ones are inactive and have value $0$.
%     The solution induces by the bold edges is feasible to constraints~\eqref{eq:lifted-disjoint-paths-problem}.
%     }
%     \label{fig:problemIllustration}
% \end{figure}

\roberto{Figure could be removed, there is nothing new after LDP..}

==> lifted disjoint paths message passing/idf1_plot.tex <==
\begin{tikzpicture}[scale=0.9]
\begin{axis}[
    title={IDF1 Ours vs. Lif\_T},
    width=0.5\textwidth,
    height=0.3\textwidth,
    xlabel={\text{Sequence length} [frames]},
    ylabel={IDF1},
    ymin=0.7, ymax=0.9,
    xmin=0, xmax=200,
    xtick={0,30,50,75,100, 125, 150,200},
    ytick={0.7,0.8,0.9},
    legend pos=north west,
    ymajorgrids=true,
    grid style=dashed,
    log ticks with fixed point,
    x tick label style={/pgf/number format/1000 sep=\,},
    legend style={at={(0.42,0.18)},anchor=west},
    legend columns=2
]

\addplot[
    color=green,
    mark=square,
    ]
    coordinates {
    (30,0.852)(50,0.833)(75,0.826)(100,0.825)(150,0.81)(200,0.754)
    };

\addplot[
    color=blue,
    mark=square,
    ]
    coordinates {
    (30,0.852)(50,0.833)(75,0.826)(100,0.825)(150,0.81)(200,0.754)
    };

\addplot[
    color=orange,
    mark=square,
    ]
    coordinates {
    (30,0.852)(50,0.815)(75,0.816)(100,0.816)(150,0.798)(200,0.746)

    };

\addplot[
    color=red,
    mark=square,
    ]
    coordinates {
    (30,0.846)(50,0.806)(75,0.794)(100,0.804)(150,0.781)(200,0.732)
    };
    \legend{Ours-6,Ours-11,Ours-31, Gurobi}
    
\end{axis}
\end{tikzpicture}

==> lifted disjoint paths message passing/include.tex <==
 \usepackage{amsthm}
% \usepackage{amsmath,amssymb} % define this before the line numbering.
% \usepackage[T1]{fontenc}
% \usepackage{etex}
% %\usepackage{graphicx}
% \usepackage{amsxtra}
% \usepackage{amsfonts}
% \usepackage{nicefrac}
% \usepackage{microtype}
 \usepackage{url}
% \usepackage{soul}
% \usepackage{todonotes}

%  \usepackage{color}
  \usepackage{bbm}
% % \usepackage{pgfplots}

\usepackage{varwidth}

% \usepackage{wrapfig}
% \usepackage{sidecap}
% %\usepackage[ruled]{algorithm2e}

% \usepackage{colortbl}
% \newcolumntype{g}{>{\columncolor[gray]{0.85}}c}

 \usepackage{epsfig}
% \usepackage{stmaryrd} % for Iverson brackets
\usepackage{mathtools}

\usepackage[bb=boondox]{mathalfa}

 \usepackage{multirow}
% \usepackage{fixmath}
 \usepackage{booktabs}
 \usepackage{comment}
% \usepackage{pbox}
% \usepackage{enumerate}
% \usepackage{enumitem}

\usepackage{algorithm}
\usepackage{algpseudocode}
\algnewcommand{\IIf}[1]{\State\algorithmicif\ #1\ \algorithmicthen}
\algnewcommand{\EElse}{\State\algorithmicelse\ }
\algnewcommand{\EndIIf}{\unskip\ \algorithmicend\ \algorithmicif}

  \usepackage{times}
  \usepackage{tabularx}
 % \usepackage{afterpage}
%  \usepackage{ulem}
%  \usepackage{placeins}
%  \usepackage{longtable}
% %%\usepackage{algpseudocode}
% %\usepackage{algorithm}
% % \usepackage{subcaption}
%  \usepackage{thmtools}
%  \usepackage{thm-restate}
%  %\usepackage{csvsimple,siunitx,booktabs,array}
% % 
% \usepackage{tikz}
% \usetikzlibrary{positioning}
% \usetikzlibrary{decorations.markings}
% % 
%  \newcommand{\MC}{\mathsf{MC}}
%  \newcommand{\re}{\mathcal{R}}
%  \newcommand{\unre}{\bar{\mathcal{R}}}

%  \setitemize{topsep=2.5pt,parsep=1.5pt,partopsep=1.5pt,leftmargin=0.4cm}
% % %\usepackage{bibspacing}
% % 
%  \declaretheorem[name=Theorem]{thm}
%  \declaretheorem[name=Proposition]{prop}
% % 
%  \mathchardef\mhyphen="2D
% % 

% \makeatletter
% \newcommand\footnoteref[1]{\protected@xdef\@thefnmark{\ref{#1}}\@footnotemark}
% \makeatother



%% ONLY During draft  %% REMOVE LATER !!
\makeatletter
\@namedef{ver@everyshi.sty}{}
\makeatother
\usepackage[disable]{todonotes}
%\usepackage{todonotes}
%%% REMOVE



% %\usepackage{caption}
% %\usepackage{subcaption}
% %\captionsetup{compatibility=false}
% %\captionsetup[subfigure]{labelfont=bf}

% %\usepackage[pagebackref=true,breaklinks=true,letterpaper=true,colorlinks,bookmarks=false]{hyperref}

\newcommand{\SE}{\mathcal{E}}
\newcommand{\SX}{\mathcal{X}}
\newcommand{\Simplex}{\mathcal{S}}
\newcommand{\SI}{\Sigma}
\newcommand{\SV}{\mathcal{V}}
\newcommand{\SM}{\mathcal{M}}
\newcommand{\SP}{\mathcal{P}}
\newcommand{\SN}{\mathcal{N}}
\newcommand{\SG}{\mathcal{G}}
\newcommand{\SL}{\mathcal{L}}

\newcommand{\BF}{\mathbb{F}}
\newcommand{\BR}{\mathbb{R}}
\newcommand{\BV}{\mathbb{V}}
\newcommand{\BE}{\mathbb{E}}
\newcommand{\BG}{\mathbb{G}}
\newcommand{\BS}{\mathbb{S}}

\newcommand{\FG}{\mathsf{G}}
\newcommand{\FV}{\mathsf{V}}
\newcommand{\FE}{\mathsf{E}}
\newcommand{\FL}{\mathsf{L}}
\newcommand{\IPSLP}{IRPS-LP}

\newcommand{\R}{\mathbb{R}}
\newcommand{\N}{\mathbb{N}}
\newcommand{\Z}{\mathbb{Z}}
\newcommand{\la}{\langle}
\newcommand{\ra}{\rangle}
\newcommand{\T}{\top}
\newcommand{\zero}{\mathbbmss{O}}
\newcommand{\eins}{\mathbbmss{1}}
\newcommand{\dcup}{\dot{\cup}}
\newcommand{\fdots}{\makebox[0.75em][c]{.\hfill.}\thinspace} % two dots to save space


\DeclareMathOperator*{\argmin}{arg min}
\DeclareMathOperator*{\argmax}{arg max}
\DeclareMathOperator*{\conv}{conv}
 \mathchardef\mhyphen="2D
 
\newcommand{\pluseq}{\mathrel{{+}{=}}}
\newcommand{\minuseq}{\mathrel{{-}{=}}}
\newcommand{\plusplus}{\mathrel{{+}{+}}}

% \def\clap#1{\hbox to 0pt{\hss#1\hss}}
% \def\mathllap{\mathpalette\mathllapinternal}
% \def\mathrlap{\mathpalette\mathrlapinternal}
% \def\mathclap{\mathpalette\mathclapinternal}
% \def\mathllapinternal#1#2{%
% \llap{$\mathsurround=0pt#1{#2}$}}
% \def\mathrlapinternal#1#2{%
% \rlap{$\mathsurround=0pt#1{#2}$}}
% \def\mathclapinternal#1#2{%
% \clap{$\mathsurround=0pt#1{#2}$}}

\providecommand{\abs}[1]{\lvert#1\rvert}
\providecommand{\norm}[1]{\lVert#1\rVert}

% \definecolor{fettrot}{RGB}{255,10,10}
% \newcommand{\todo}[1]{\colorbox{fettrot}{TODO: \color{black}#1}}

\newtheorem{example}{Example}
\newtheorem{definition}{Definition}
\newtheorem{theorem}{Theorem}
\newtheorem{lemma}{Lemma}
\newtheorem{proposition}{Proposition}
\newtheorem{remark}{Remark}



% \usepackage{tikz}
% \usetikzlibrary{arrows}
%  %   \definecolor{joincolor}{HTML}{000000}
%     \usetikzlibrary{decorations.pathmorphing}
%     \tikzstyle{lifted-edge}=[->,> = latex',blue]
%     \tikzstyle{base-edge}=[->,> = latex',black]
% 	\tikzstyle{cut-edge}=[->,> = latex',dashed]
%     \tikzstyle{vertex}=[circle, draw, inner sep=0pt,text height=3mm,text width=3mm,text depth=1.5mm,align=center]
%     % \tikzstyle{vertex}=[circle, draw, fill=white, inner sep=0.1pt,minimum width=1ex, maximum width=4cm]
%   \tikzset{every picture/.append style={baseline,scale=1.1}}


==> lifted disjoint paths message passing/introduction.tex <==
\section{Introduction}
\andrea{Should we include MOT16 and MOT15 in the abstract? Can we replace solvers (plural) by solver?}
\timo{i think we should}

% Why is MOT important in general ? 
Deriving high-level understanding from a video is a desired task that has been studied in computer vision for a long time. Nevertheless, solving the problem is a long way off.
A computer vision system able to extract the motions of objects appearing in a video  in terms of trajectories is considered as a prerequisite for the goal. This task, called multiple object tracking (MOT), has numerous applications, e.g.\ in the area of video surveillance~\cite{fenzi2014asev}, sports analysis~\cite{alahi2009sport,lu2013learning}, urban planning~\cite{alahi2017unsupervised}, or autonomous driving~\cite{liang2020pnpnet,frossard2018end}. 

Yet, solving MOT is challenging, especially for long and crowded sequences.
% How is MOT approached ? 
The predominant approach for MOT is the tracking-by-detection paradigm, which splits the problem into two subtasks. First, objects are detected in all video frames by an object detector. Then, the detections are linked across frames to form trajectories. While the performance of object detectors has improved considerably by recent advances of CNNs \cite{ren2015faster,yang2016exploit,redmon2016you,duan2019centernet}, the latter task called the  \textit{data association} remains challenging. 
The data association reasons from \textit{pairwise costs},  which indicate for each pair of detections the likelihood of belonging to the same object.
%Why is the data association problem difficult  w.r.t inputs? 

Appearance and spatio-temporal information are often ambiguous, especially in crowded scenes and pairwise costs can be misleading. Moreover, object detectors produce more errors in crowded scenes due to partial occlusions.
To resolve these issues, it is crucial that the data association incorporates global context.

% How is the data association solved ? 
The disjoint paths problem (DP)~\cite{zhang2008global,kovacs2015minimum} is a natural model for MOT. Results are computed efficiently  using a min-cost flow algorithm that delivers the global optimal solution. 
Unfortunately, the integration of long range temporal interactions is limited, as DP obeys the first-order Markov-chain assumption: for each trajectory, consistency is ensured only between directly linked detections, which is a strong simplification that ignores higher order consistencies among multiple linked detections.

%\begin{figure}[t]
%\include{runtime_plot}
%\caption{Runtime comparison between Ours with 6, 11 and 31 iterations against globally optimal Gurobi\cite{gurobi}. For the comparison we clipped the complex tracking sequence \textit{MOT20-01} from MOT20 dataset\cite{MOTChallenge20} after several numbers of frames to measure the runtime with subject to increasing problem complexity.}
%\label{fig:runtime}
%\end{figure}

% How can this deficiency be fixed ?
% To fix this deficiency, the disjoint paths  problem has been generalized to the lifted disjoint paths (LDP) \cite{hornakova2020lifted}, where additional connectivity priors (in terms of \textit{lifted} edges) are added, making the formulation much more expressive while maintaining the feasibility set of the DP formulation, see Section \ref{sec:problem_formulation}. 
% The optimization problem then  takes all connections within a trajectory into account (in terms of the pairwise costs). It thus enables to incorporate long range temporal interactions effectively, which  has been shown to improve recall and precision considerably  \cite{hornakova2020lifted}. Similar extensions have been made for the multicut problem \cite{tang2016multi,tang2017multiple}.

To fix this deficiency, \cite{hornakova2020lifted}  generalizes DP to lifted disjoint paths (LDP) by using additional connectivity priors in terms of \textit{lifted} edges. This makes the formulation much more expressive while it maintains the feasibility set of the DP (Sec.\ \ref{sec:problem_formulation}). 
The optimization problem enables to take  into account pairwise costs between arbitrary detections belonging to one trajectory. It thus enables to incorporate long range temporal interactions effectively and leads to considerable improvement of recall and precision  \cite{hornakova2020lifted}. Similar extensions have been made for the multicut problem \cite{tang2016multi,tang2017multiple}.


While the integration of the global context by LDP is crucial to obtain high-quality tracking results,  it makes  the data association problem  NP-hard.
%, and the set of feasible trajectories  has exponential growth.
Still, \cite{hornakova2020lifted} presented a~global optimal LDP solver usable for  semi-crowded sequences with reasonable computational effort.
However, when applied to  longer and crowded sequences, such approaches are not tractable anymore, due to too high demands on runtime and memory.
\andrea{Shall we use LDP solver instead of solvers? There is only one solver, right?}
\roberto{We can do it, but then consistent with the abstract}

In order to close this gap, we present the first approximate solver for LDP.
The resulting tracker scales to big problem instances and incorporates global context with similar accuracy as the global optimal LDP solver.
Moreover, our solver outputs certificates in terms of primal/dual gaps.
%While being approximative, the solver still outputs certificates in terms of primal/dual gaps and relies on a convex relaxation, hence still being a principled algorithm.

In particular, our solver is based on a Lagrangean (dual) decomposition of the problem.
This dual is iteratively optimized by dual block coordinate ascent (a.k.a.\ message passing) using techniques from~\cite{Swoboda_2017_CVPR}, see Sec.~\ref{sec:lagrange-decomposition-sub}.
The decomposition relies on subproblems that are added in a cutting plane fashion.
We obtain high-quality primal solutions by solving minimum cost flow problems with edge costs synthesizing information from both base and lifted edges from the dual task and improve them via a local search procedure. 
%Moreover, the costs are estimated on lightweight features to reduce computational efforts for large and dense datasets.
%Additional to the efficient solver the costs are estimated on lightweight features to reduce computational efforts for large and dense datasets. 



 
% We validate the approximating quality of solver on several state-of-the-art MOT benchmarks in Section \ref{sec:experiments}. It achieves \textcolor{blue}{comparable or better} performance as the current state of the art on MOT15\cite{MOTChallenge2015}, MOT16 and MOT17\cite{MOT16}, which are datasets known to be already saturating \cite{hornakova2020lifted}.

%We show that our solver achieves state-of-the-art performance on the MOT17 dataset \cite{?}, which consists of semi-crowded sequences. In particular, the results are on pair with the results obtained by exchanging our solver with an optimal LDP solver. 
We validate the quality of the solver on four standard MOT benchmarks (Sec.~\ref{sec:experiments}). We achieve comparable or better performance w.r.t.\ the current state-of-the-art trackers including the tracker based on the  optimal LDP solver~\cite{hornakova2020lifted} on MOT15/16/17~\cite{MOTChallenge2015,MOT16}.
Furthermore, our proposed tracker performs on par with state-of-the-art on the more challenging MOT20 dataset~\cite{MOTChallenge20} which is composed of long and crowded sequences. Lightweight features and a fast solver are crucial to perform tracking on such massive sequences.
%
%Due to the high density of objects, the extension LDP-based methods requires lightweight features and a fast solver. 
Our work thus extends the applicability of the successful LDP formulation to a wider range of  instances.

\myparagraph{Contribution} of this work is in summary as follows:
%\noindent In summary, the contribution of this work is as follows:
\noindent\begin{itemize}
%   \setlength{\parskip}{0pt}
%   \setlength{\itemsep}{0pt}
%   \setlength{\leftmargin}{0cm}
%   \setlength{\topsep}{0pt}
%   \setlength{\partopsep}{0pt}
    \item We make the LDP problem more accessible and applicable by introducing an approximate solver with better scalability properties than the global optimal LDP solver, while resulting in similar tracking performance, and being independent of Gurobi \cite{gurobi}. 
    \item We present an MOT system that is scalable to challenging sequences by using considerably less computationally demanding features than what is used in the state-of-the-art tracker \cite{hornakova2020lifted}. Our system %is the first to
    incorporates higher order consistencies in a scalable way, i.e.\ it uses an approximate solver and provides  a~gap to the optimum. 
   % \item Fast Convergence..
    
\end{itemize}
 We make our LDP solver\footnote{\url{https://github.com/LPMP/LPMP}} and our MOT pipeline\footnote{\url{https://github.com/TimoK93/ApLift}} available.




==> lifted disjoint paths message passing/mot17train.tex <==
\begin{table*}
\center
\small{
%\caption{LDP solver runtime and IDF1 comparison between our solver with 6, 11, 31, 51 and 101 iterations against globally optimal
\caption{Runtime and IDF1 comparison of LDP solvers: ApLift (ours)  with 6, 11, 31, 51 and 101 iterations and globally optimal (one step)
LifT\cite{hornakova2020lifted} on MOT17 train. Numbers in parenthesis in the time column show the difference between the solvers, in the IDF1 column the ratio between Lift and ApLift.}
\label{tabel:runtimeMOT17}
\begin{tabular}{l  c c  c c  c c  c c  c c  c c}
%\cline{1-7}
\toprule
 & \multicolumn{2}{c}{LifT} & \multicolumn{2}{c}{Ours-6} & \multicolumn{2}{c}{Ours-11} & \multicolumn{2}{c}{Ours-31} & \multicolumn{2}{c}{Ours-51} & \multicolumn{2}{c}{Ours-101}\\
Sequence Name & Time$\downarrow$ & IDF1$\uparrow$ & Time$\downarrow$ & IDF1$\uparrow$ & Time$\downarrow$ & IDF1$\uparrow$ & Time$\downarrow$ & IDF1$\uparrow$ & Time$\downarrow$ & IDF1$\uparrow$ & Time$\downarrow$ & IDF1$\uparrow$\\ \toprule
\multirow{2}{*}{02-DPM} &$ 7324 $&$ \textbf{49.4} $&$ 94 $&$ 47.4 $&$ 157 $&$ 47.4 $&$ 513 $&$ 49.1 $&$ 989 $&$ 49.1 $&$ 2415 $&$ 49.1 $\\
 &$ (1.0) $&$ (0.0) $&$ (0.01) $&$ (-2.00) $&$ (0.02) $&$ (-2.00) $&$ (0.07) $&$ (-0.30) $&$ (0.14) $&$ (-0.30) $&$ (0.33) $&$ (-0.30)$ \\  \midrule
\multirow{2}{*}{02-FRCNN} &$ 4073 $&$ 54.7 $&$ 97 $&$ \mathbf{54.9 }$&$ 161 $&$ \mathbf{54.9 } $&$ 526 $&$ \mathbf{54.9 } $&$ 1021 $&$ \mathbf{54.9 } $&$ 2503 $&$ \mathbf{54.9 } $\\
 &$ (1.0) $&$ (0.0) $&$ (0.02) $&$ (0.20) $&$ (0.04) $&$ (0.20) $&$ (0.13) $&$ (0.20) $&$ (0.25) $&$ (0.20) $&$ (0.61) $&$ (0.20)$ \\  \midrule
\multirow{2}{*}{02-SDP} &$ 7795 $&$ \mathbf{56.7} $&$ 131 $&$ 55.0 $&$ 219 $&$ 55.0 $&$ 717 $&$ 55.0 $&$ 1410 $&$ 55.0 $&$ 3685 $&$ 55.0 $\\
 &$ (1.0) $&$ (0.0) $&$ (0.02) $&$ (-1.70) $&$ (0.03) $&$ (-1.70) $&$ (0.09) $&$ (-1.70) $&$ (0.18) $&$ (-1.70) $&$ (0.47) $&$ (-1.70)$ \\  \midrule
\multirow{2}{*}{04-DPM} &$ * $&$ \mathbf{75.4} $&$ 449 $&$ 74.7 $&$ 756 $&$ 74.7 $&$ 2220 $&$ 74.7 $&$ 3929 $&$ 75.0 $&$ 8578 $&$ 75.0 $\\
 &$ (*) $&$ (0.0) $&$ (*) $&$ (-0.70) $&$ (*) $&$ (-0.70) $&$ (*) $&$ (-0.70) $&$ (*) $&$ (-0.40) $&$ (*) $&$ (-0.40)$ \\  \midrule
\multirow{2}{*}{04-FRCNN} &$ 4889 $&$ \mathbf{79.2} $&$ 383 $&$ 78.1 $&$ 644 $&$ 78.1 $&$ 1811 $&$ 76.3 $&$ 3111 $&$ 78.2 $&$ 6565 $&$ 78.2$ \\
 &$ (1.0) $&$ (0.0) $&$ (0.08) $&$ (-1.10) $&$ (0.13) $&$ (-1.10) $&$ (0.37) $&$ (-2.90) $&$ (0.64) $&$ (-1.00) $&$ (1.34) $&$ (-1.00)$ \\  \midrule
\multirow{2}{*}{04-SDP} &$ * $&$ \mathbf{82.3} $&$ 499 $&$ 78.0 $&$ 839 $&$ 78.0 $&$ 2441 $&$ 78.0 $&$ 4294 $&$ 77.7 $&$ 9269 $&$ 79.9 $\\
 &$ (*) $&$ (0.0) $&$ (*) $&$ (-4.30) $&$ (*) $&$ (-4.30) $&$ (*) $&$ (-4.30) $&$ (*) $&$ (-4.60) $&$ (*) $&$ (-2.40) $\\  \midrule
\multirow{2}{*}{05-DPM} &$ 535 $&$ \mathbf{65.0} $&$ 10 $&$ 62.6 $&$ 15 $&$ 62.6 $&$ 57 $&$ 63.5 $&$ 116 $&$ 63.5 $&$ 298 $&$ 63.5$ \\
 &$ (1.0) $&$ (0.0) $&$ (0.02) $&$ (-2.40) $&$ (0.03) $&$ (-2.40) $&$ (0.11) $&$ (-1.50) $&$ (0.22) $&$ (-1.50) $&$ (0.56) $&$ (-1.50)$ \\  \midrule
\multirow{2}{*}{05-FRCNN} &$ 514 $&$ \mathbf{66.6} $&$ 10 $&$ 63.8 $&$ 15 $&$ 63.8 $&$ 57 $&$ 64.0 $&$ 118 $&$ 63.9 $&$ 315 $&$ 65.6 $\\
 &$ (1.0) $&$ (0.0) $&$ (0.02) $&$ (-2.80) $&$ (0.03) $&$ (-2.80) $&$ (0.11) $&$ (-2.60) $&$ (0.23) $&$ (-2.70) $&$ (0.61) $&$ (-1.00) $\\  \midrule
\multirow{2}{*}{05-SDP} &$ 604 $&$ \mathbf{67.9} $&$ 11 $&$ \mathbf{67.9} $&$ 18 $&$ \mathbf{67.9} $&$ 67 $&$ 67.1 $&$ 137 $&$ 67.1 $&$ 364 $&$ 67.6 $\\
 &$ (1.0) $&$ (0.0) $&$ (0.02) $&$ (0.00) $&$ (0.03) $&$ (0.00) $&$ (0.11) $&$ (-0.80) $&$ (0.23) $&$ (-0.80) $&$ (0.60) $&$ (-0.30) $\\  \midrule
\multirow{2}{*}{09-DPM} &$ 6692 $&$ \mathbf{67.5} $&$ 42 $&$ 66.4 $&$ 70 $&$ 66.4 $&$ 232 $&$ \mathbf{67.5} $&$ 480 $&$ \mathbf{67.5} $&$ 1281 $&$ \mathbf{67.5} $\\
 &$ (1.0) $&$ (0.0) $&$ (0.01) $&$ (-1.10) $&$ (0.01) $&$ (-1.10) $&$ (0.03) $&$ (0.00) $&$ (0.07) $&$ (0.00) $&$ (0.19) $&$ (0.00) $\\  \midrule
\multirow{2}{*}{09-FRCNN} &$ 11888 $&$ \mathbf{68.2} $&$ 37 $&$ \mathbf{68.2} $&$ 61 $&$ \mathbf{68.2} $&$ 201 $&$ \mathbf{68.2} $&$ 407 $&$ \mathbf{68.2} $&$ 1095 $&$ \mathbf{68.2} $\\
 &$ (1.0) $&$ (0.0) $&$ (0.00) $&$ (0.00) $&$ (0.01) $&$ (0.00) $&$ (0.02) $&$ (0.00) $&$ (0.03) $&$ (0.00) $&$ (0.09) $&$ (0.00) $\\  \midrule
\multirow{2}{*}{09-SDP} &$ 1462 $&$ \mathbf{68.6} $&$ 44 $&$ 67.1 $&$ 74 $&$ 67.1 $&$ 247 $&$ 68.5 $&$ 512 $&$ 68.5 $&$ 1443 $&$ 68.5 $\\
 &$ (1.0) $&$ (0.0) $&$ (0.03) $&$ (-1.50) $&$ (0.05) $&$ (-1.50) $&$ (0.17) $&$ (-0.10) $&$ (0.35) $&$ (-0.10) $&$ (0.99) $&$ (-0.10) $\\  \midrule
\multirow{2}{*}{10-DPM} &$ * $&$ 66.0 $&$ 279 $&$ \mathbf{68.0} $&$ 466 $&$ \mathbf{68.0} $&$ 1524 $&$ 66.8 $&$ 3087 $&$ 67.0 $&$ 9478 $&$ 67.9 $\\
 &$ (*) $&$ (0.0) $&$ (*) $&$ (2.00) $&$ (*) $&$ (2.00) $&$ (*) $&$ (0.80) $&$ (*) $&$ (1.00) $&$ (*) $&$ (1.90) $\\  \midrule
\multirow{2}{*}{10-FRCNN} &$ * $&$ 65.2 $&$ 310 $&$ 68.8 $&$ 511 $&$ 68.5 $&$ 1689 $&$ \mathbf{69.4 }$&$ 3428 $&$ \mathbf{69.4 } $&$ 10743 $&$ \mathbf{69.4 } $\\
 &$ (*) $&$ (0.0) $&$ (*) $&$ (3.60) $&$ (*) $&$ (3.30) $&$ (*) $&$ (4.20) $&$ (*) $&$ (4.20) $&$ (*) $&$ (4.20) $\\  \midrule
\multirow{2}{*}{10-SDP} &$ * $&$ 65.4 $&$ 379 $&$ 67.0 $&$ 630 $&$ 67.0 $&$ 2090 $&$ 67.4 $&$ 4294 $&$ 67.1 $&$ 13379 $&$ \mathbf{69.8} $\\
 &$ (*) $&$ (0.0) $&$ (*) $&$ (1.60) $&$ (*) $&$ (1.60) $&$ (*) $&$ (2.00) $&$ (*) $&$ (1.70) $&$ (*) $&$ (4.40) $\\  \midrule
\multirow{2}{*}{11-DPM} &$ 1991 $&$ \mathbf{76.3} $&$ 60 $&$ \mathbf{76.3} $&$ 99 $&$ \mathbf{76.3} $&$ 335 $&$\mathbf{76.3} $&$ 672 $&$ \mathbf{76.3} $&$ 1672 $&$ \mathbf{76.3} $\\
 &$ (1.0) $&$ (0.0) $&$ (0.03) $&$ (0.00) $&$ (0.05) $&$ (0.00) $&$ (0.17) $&$ (0.00) $&$ (0.34) $&$ (0.00) $&$ (0.84) $&$ (0.00) $\\  \midrule
\multirow{2}{*}{11-FRCNN} &$ 2382 $&$ \mathbf{78.3} $&$ 68 $&$ \mathbf{78.3} $&$ 113 $&$ \mathbf{78.3} $&$ 366 $&$ \mathbf{78.3} $&$ 729 $&$ \mathbf{78.3} $&$ 1799 $&$ \mathbf{78.3} $\\
 &$ (1.0) $&$ (0.0) $&$ (0.03) $&$ (0.00) $&$ (0.05) $&$ (0.00) $&$ (0.15) $&$ (0.00) $&$ (0.31) $&$ (0.00) $&$ (0.76) $&$ (0.00) $\\  \midrule
\multirow{2}{*}{11-SDP} &$ 3195 $&$ 80.0 $&$ 68 $&$ 79.8 $&$ 113 $&$ 79.8 $&$ 370 $&$ \mathbf{80.1} $&$ 748 $&$ 80.0 $&$ 2057 $&$ 80.0 $\\
 &$ (1.0) $&$ (0.0) $&$ (0.02) $&$ (-0.20) $&$ (0.04) $&$ (-0.20) $&$ (0.12) $&$ (0.10) $&$ (0.23) $&$ (0.00) $&$ (0.64) $&$ (0.00) $\\  \midrule
\multirow{2}{*}{13-DPM} &$ * $&$ 62.8 $&$ 152 $&$ \mathbf{66.8} $&$ 252 $&$ \mathbf{66.8} $&$ 944 $&$ \mathbf{66.8} $&$ 2008 $&$ \mathbf{66.8} $&$ 6340 $&$ 65.7 $\\
 &$ (*) $&$ (0.0) $&$ (*) $&$ (4.00) $&$ (*) $&$ (4.00) $&$ (*) $&$ (4.00) $&$ (*) $&$ (4.00) $&$ (*) $&$ (2.90) $\\  \midrule
\multirow{2}{*}{13-FRCNN} &$ * $&$ 62.5 $&$ 217 $&$ \mathbf{69.8} $&$ 351 $&$ \mathbf{69.8} $&$ 1331 $&$\mathbf{69.8} $&$ 2942 $&$ 67.7 $&$ 9813 $&$ 66.2 $\\
 &$ (*) $&$ (0.0) $&$ (*) $&$ (7.30) $&$ (*) $&$ (7.30) $&$ (*) $&$ (7.30) $&$ (*) $&$ (5.20) $&$ (*) $&$ (3.70) $\\  \midrule
\multirow{2}{*}{13-SDP} &$ * $&$ 64.5 $&$ 196 $&$ \mathbf{66.8} $&$ 326 $&$ \mathbf{66.8} $&$ 1237 $&$ \mathbf{66.8} $&$ 2698 $&$ 66.2 $&$ 8954 $&$ 65.6 $\\
 &$ (*) $&$ (0.0) $&$ (*) $&$ (2.30) $&$ (*) $&$ (2.30) $&$ (*) $&$ (2.30) $&$ (*) $&$ (1.70) $&$ (*) $&$ (1.10) $\\  \midrule
\multirow{2}{*}{OVERALL} &$ * $&$ \mathbf{70.7} $&$ 168 $&$ 70.3 $&$ 280 $&$ 70.3 $&$ 904 $&$ 70.2 $&$ 1768 $&$ 70.3 $&$ 4859 $&$ \mathbf{70.7} $\\
 &$ (*) $&$ (0.0) $&$ (*) $&$ (-0.40) $&$ (*) $&$ (-0.40) $&$ (*) $&$ (-0.50) $&$ (*) $&$ (-0.40) $&$ (*) $&$ (0.00) $\\  \bottomrule
\end{tabular}
}
\end{table*}


==> lifted disjoint paths message passing/relatedWork.tex <==
\section{Related Work}
% TODO: Paul: write combinatorial, contribution, line 246 (approximate solver characteristics, advantages)
% \begin{itemize}
%     \item Lift (better scaling in terms of speed, while same accuracy. Crucial for crowded scenes like in MOT20)
%     \item Correlation clustering trackers. They all use non-optimal solvers. Why this approach is superior..
%     \item Graph Message passing for tracking (higher order solved heuristically by the graph neural network). We have principled formulation for HO
%     \item Tracking-by-regression (BellsWhistles): basis of our work. But only to obtain detections. Tracking-by-regression accuracy worse compared to offline approaches.
% \end{itemize}

%\todo[inline]{Regarding MOT related work: I would suggest one or two paragraphs for MOT. I would say something similar to the lift paper: \textbf{Solving MOT with Connectivity priors \& lifted edges} and \textbf{Other  combinatorial  approaches  to  MOT.}.}


%\myparagraph{Message passing} in tracking is used to aggregate higher order (HO) information. In \cite{braso2020learning} Graph Neural Networks update initial link probabilities between object detections which approximately solves the binary association problem. Other works \cite{9007500} formulate the MOT problem as a conditional random field graph and pass HO information during iterative minimization of a global objective. [... to be continued]

%\myparagraph{Tracking-by-Regression} as coined in \cite{dendorfer2020tracking} solves the MOT problem by tracking single targets mostly independent. Target tracks are initiated by an object detector and updated by regression. Thus, these methods are only partly depending on object detection quality, but are limited in using higher order information. They are ignored or implicitly used in motion/appearance models like in \cite{10.1007/978-3-319-46448-0_45}. However, regression-based methods archive SOTA performance \cite{bergmann2019tracking, 10.1007/978-3-030-58548-8_28}. This work uses detections generated by a regression-based SOTA method to be comparable.


% \myparagraph{(Lifted) Disjoint Path.}
% Quickly recap disjoint path tracking to make advantage of lifted DP  clear.
% Recap quickly advantage of lifted formulation w.r.t MOT, e.g leading to very good results by incoroporating long-term information. Problem is NP-hard.
% Only available solver is global optimal, thus not scalable.
% This work presents an approximative solver for Lift.

\myparagraph{(Lifted) disjoint paths. }The disjoint paths problem is a natural model for multiple object tracking and is solvable with fast combinatorial solvers~\cite{kovacs2015minimum}. It has been used for the data association step of MOT in~\cite{berclaz2011multiple,zhang2008global}. Its extensions  have been used for fusing different object detectors~\cite{chari2015pairwise} or multi-camera MOT~\cite{hofmann2013hypergraphs,leal2012branch}. Its main disadvantage is that it does not allow to integrate long range information because it evaluates only direct connections between object detections within a trajectory.
The lifted disjoint paths problem introduced in~\cite{hornakova2020lifted} enhances DP by introducing lifted edges that enable to reward or penalize arbitrary connections between object detections. This incorporation of long range information leads to a significant improvement of the tracking performance yielding state-of-the-art results on main MOT benchmark but makes the problem NP-hard. The authors provide a globally optimal solver using Gurobi~\cite{gurobi}. Despite a lot of efficient subroutines, the general time complexity of the provided solver remains exponential.
Therefore, in order to extend LDP-based methods to highly dense MOT problems as in MOT20 it is crucial to reduce the complexity of the used LDP solver
because the number of feasible connections between detections increases dramatically.
%due to the dramatically increasing number of feasible connections between detection.
%due to the dramatically increasing feasible connections between detections.
%The extension of LDP-based methods to highly dense MOT problems as in MOT20 is crucial due to the dramatically increasing feasible connections between detections. 
%Lifted disjoint paths problem introduced in~\cite{hornakova2020lifted}  incorporates long range information into the disjoint paths formulation by introducing lifted edges that enable to reward or penalize arbitrary connections between detections.  This incorporation of long range information leads to a significant improvement of tracking performance.


% \myparagraph{Other data association approaches for MOT.}

% \begin{itemize}
%     \item Shortly mention Bells and Whistles \cite{bergmann2019tracking} and CenterTrack \cite{zhou2020tracking}. They effectively recovers missing detections but employs a greedy (Bells and Whistles) and limited (CenterTrack frame-to-frame)  data association strategy, thus being prone to ID switches and suffer from long-term occlusions. Applying BnW to a sequence builds the basis for our tracker. 
%     \item Learning a neural solver \cite{braso2020learning}. Long term information are implicitly processed via graph message passing. Allows to learn features "directly" for the tracking task.
%     Disadvantages:
%     \begin{itemize}
%         \item Memory and computationally demanding as big neural network architecture is employed, modeling the input sequence (subsampling necessary).
%         \item Not directly optimizing tracking problem: Data association not enforced by the neural network (rounding necessary and flow conservation constraint not ensured). 
%     \end{itemize}
%     \item Multicut
%     \begin{itemize}
%         \item In principle. we can use most parts similiar to Lift section about MC
%         \item However, we cannot argue that the MC works employ heuristics in contrast to this work. 
%         \andrea{Message passing is better than just a heuristic because we have the lower bound. Therefore, we know what is the quality of our solution.}
%         \roberto{OK very good! Are there message passing solvers for MC or LMC ? }
%         \andrea{There is a message passing multicut solver within LPMP. It was not applied to MOT. I do not know any lifted multicut message passing solver. }
%         \item NEW: \textit{A Two-Stage Minimum Cost Multicut Approach to Self-Supervised Multiple Person Tracking}
%         \begin{itemize}
%             \item Learns pairwise features on the tracking result (cluster short tracks via MC, then update pairwise features, cluster again and iterate).
%             \item Avoids the necessity to create labels for training data. 
%             \item Could be mentioned together with MC approaches.
%         \end{itemize}
%     \end{itemize}
% \end{itemize}

\myparagraph{Multicut and lifted multicut.} LDP is similar to (lifted) multicut~\cite{chopra1993partition,hornakova2017analysis}.
Multicut has been used for MOT in ~\cite{Ho_2020_ACCV,keuper2018motion,kumar2014multiple,ristani2014tracking,tang2015subgraph,tang2016multi}, lifted multicut in~\cite{babaee2018multiple,tang2017multiple}.
%Where the work~\cite{Ho_2020_ACCV} deserves a special attention because it is a self-supervised technique that does not need labels for the training data.
These trackers solve the underlying combinatorial problem approximately via heuristics without providing an estimation of the  gap to optimality.
Our approach,  delivers an approximate solution together with a lower bound enabling to assess the quality of the solution.
Additionally, LDP provides a strictly better relaxation than lifted multicut~\cite{hornakova2020lifted}.

%Although there exists a message passing algorithm for the multicut problem within the same framework as we use~\cite{Swoboda_2017_CVPR_multicut}, it has not been applied to the MOT. 
%\roberto{Can we remove the highlight about self-supervised tracking ? Just list it with the others? }


% {\color{blue}
% \myparagraph{Other combinatorial approaches to MOT.}
% Other combinatorial approaches to MOT include maximum clique problem~\cite{zamir2012gmcp,dehghan2015gmmcp}, maximum independent set~\cite{brendel2011multiobject} and multigraph-matching problem~\cite{hu2019dual}.
% The minimum cost arborescence problem, has been used in~\cite{henschel2014efficient}.

% \andrea{@Roberto, can you please re-formulate the following text. It is now a copy from LifT paper.}
% The works~\cite{Henschel_2018_CVPR_Workshops,henschel2016tracking} reformulate tracking multiple objects with long temporal interactions as a binary quadratic program. If the problem size is small, the optimization problem can be solved optimally by reformulating it to an equivalent binary linear program \cite{henschel2020simultaneous,von2018recovering}. For large instances, an approximation is necessary.  To this end, a specialized non-convex Frank-Wolfe method can be used \cite{Henschel_2018_CVPR_Workshops}.


% }

\myparagraph{Other data association models for MOT.}
Several works employ greedy heuristics to obtain tracking results \cite{bochinski2017high,zhou2021tracking,bergmann2019tracking}.
%, \eg based on the intersection-over-union between two detections \cite{bochinski2017high}, using a neural network that detects for a given frame all objects and their predicted positions in the previous frame \cite{zhou2021tracking}, or by propagating each trajectory to the next frame using the regression head of an object detector \cite{bergmann2019tracking}.
Such strategies normally  suffer from occlusions or ambiguous situations, causing  trajectory errors. Others use bipartite matchings \cite{huang2008robust,sadeghian2017tracking,zhu2018online,xu2019spatial,Wojke2017simple,Wojke2018deep} to assign  new detections with already computed trajectories of the past optimally. Since no global context is incorporated,  they are  prone to errors if individual edge costs are misleading. %For a global view, MOT  has been formulated as minimum cost arborescence problem \cite{henschel2014efficient}, which is corresponds to the minimum spanning tree problem for directed graphs. 

Higher order MOT frameworks ensure consistencies within all detections of a trajectory.
%
This can be done greedily, by computing one trajectory at a time via  a generalized minimum clique problem \cite{zamir2012gmcp}, or globally using an  extension to the maximum multi clique problem \cite{dehghan2015gmmcp}. 

\roberto{Relating the problems to Multicut would have the advantage that the reader understand that they are NP-hard and can only be solved so far using KL heuristics..}

%Several works approximate the tracking solution in the continuous domain.
Several works employ continuous domain relaxation.
When MOT is formulated as a binary quadratic program \cite{Henschel_2018_CVPR_Workshops,henschel2019multiple,von2018recovering,henschel2020simultaneous}, a modification of the Frank-Wolfe algorithm adapted to the non-convex case has been used  \cite{Henschel_2018_CVPR_Workshops}. 
%This enables to solve big problem instances \cite{Henschel_2018_CVPR_Workshops,henschel2019multiple}. If the number of objects to be tracked is small, the problem can be solved to optimality using a reformulation as an equivalent binary linear program  \cite{von2018recovering,henschel2020simultaneous}. 
Some approximations for binary linear programs use an LP-relaxation, optimize in the continuous domain and derive a~binary solution from the continuous one \cite{jiang2007linear,chari2015pairwise,brendel2011multiobject}.
They however do not provide the optimality gap, in contrast to our work.
Higher order MOT can be considered as a classification problem using graph convolutions \cite{braso2020learning}.
It allows to train features directly on the tracking task.
%Trajectories are obtained from the continuous domain. 
%Methods operating in the continuous domain are prone to get stuck in a local optimum (in the continuous domain) and do not provide optimality certificates, in contrast to our work. 


The multigraph-matching problem, a generalization of the graph matching problem, has been used  for MOT \cite{hu2019dual}.
Here, cycle consistency constraints of the multi-graph matching ensures higher order consistencies of the trajectories.
Message passing for higher order matching in MOT has been used in~\cite{aroraICCV13}
employing a~variant of MPLP~\cite{globerson2007fixing}.
In contrast to our formulation,~\cite{aroraICCV13} does not model occlusions and does not allow for connectivity priors.

Probabilistic approaches to multiple-target tracking include multiple hypotheses tracking~\cite{kim2015multiple,chong2018forty}, joint probabiblistic data association~\cite{rezatofighi2015joint,9011349} and others  \cite{9011349,meyer2018message}.
% Finally, multiple hypothesis tracker assign each feasible trajectory a weight. Solving the underlaying maximum weight independent set problem \cite{brendel2011multiobject,kim2015multiple} relies on aggressive pruning strategies \cite{kim2015multiple} or LP-relaxation \cite{brendel2011multiobject}.  

% \textcolor{blue}{Finally, multiple hypothesis tracker assign each feasible trajectory (instead of a pair of detections) a weight. Solving the underlaying maximum weight independent set problem \cite{brendel2011multiobject,kim2015multiple} relies on aggressive pruning strategies \cite{kim2015multiple} to reduce the search space, or to approximate the problem using a LP-relaxation \cite{brendel2011multiobject}.}  
\roberto{Paul wrote its the same as a maximum clique on the complement graph. Should I mention that? -> no}
\timo{I would like to remove it}


% \begin{itemize}
%     %\item MCA \cite{henschel2014efficient}
%     %\item Minimum clique \cite{dehghan2015gmmcp,zamir2012gmcp} (GMCP, GMMCP)
%     %\item Maximum weight independent set \cite{chen2017enhancing,brendel2011multiobject}   (guarantee to a local maximum, solved on the contineous domain)
%     \item BQP \cite{Henschel_2018_CVPR_Workshops,henschel2019multiple}
%     \item CRF \cite{}
%     \item
%     \item Graph Matching \cite{hu2019dual}
%     \item Bipartite Graph Matching 
%     %\item MHT \cite{kim2015multiple}
%     %\item Greedy \cite{bergmann2019tracking} (Tracktor), Centertrack \cite{zhou2021tracking}, IOU-Greedy 
%     \item Graph Message passing \cite{braso2020learning} (Classification problem) (HO Tracking)
% \end{itemize}








\begin{comment}
\textcolor{red}{Text copied from LifT paper}

{\color{gray}\myparagraph{Disjoint paths problem.} I WOULD LEAVE THIS OUT.
The disjoint paths problem 
can be solved with fast combinatorial solvers~\cite{kovacs2015minimum}. 
The shortest paths method for network flow specialized for the disjoint paths problem~\cite{wang2019mussp} performs extremely well in practice.
For the case of the two disjoint paths problem the specialized combinatorial algorithm by Suurballe's~\cite{suurballe1974disjoint} can be used.
%

There exist several NP-complete extensions to the disjoint paths problem.
The shortest disjoint paths problem with multiple source-sink pairs~\cite{eilam1998disjoint} is NP-complete, as is the more general integer multicommodity flow problem~\cite{EvenMulti}.
The special case of the disjoint paths problem with two distinct source/sink pairs can be solved in polynomial time, however~\cite{tholey2012linear}.
}

\myparagraph{Connectivity priors \& lifted edges.}
For several combinatorial problems, special connectivity inducing edges, which we will call lifted edges for our problem, have been introduced to improve expressiveness of the  base problem.

In the Markov Random Field literature, special connectivity inducing edges were studied from a polyhedral point of view in~\cite{nowozin2010global}.
They were used in image analysis to indicate that two non-adjacent pixels come from the same object and hence they must be part of a contiguously labeled component of the underlying graph.

For multicut (a.k.a.\ correlation clustering), a classical graph decomposition problem, lifted edges have been introduced in~\cite{keuper2015lifted} to model connectivity priors. 
A lifted edge expresses affinity of two nodes to be in the same/different connected component of the graph partition.
%
Lifted multicut has been used for image and mesh segmentation~\cite{keuper2015lifted}, connectomics~\cite{beier2017multicut} and cell tracking~\cite{rempfler2017efficient}.
A combination of the lifted multicut problem and Markov Random Fields has been proposed in~\cite{levinkov2017joint} with applications in instance-separating semantic segmentation~\cite{kirillov2017instancecut}.
A polyhedral study of lifted multicut was presented in~\cite{hornakova2017analysis}.

Yet, for the above problems, global optimization  has only been reported for small instances.

{\color{gray}
\myparagraph{Disjoint paths for MOT.} DONE.
The data association step of MOT has been approached using the disjoint path setup ~\cite{berclaz2011multiple,zhang2008global}, since disjoint paths through a graph naturally model trajectories of multiple objects. 
Extension of the plain disjoint paths problem that disallow certain pairs of detections to occur simultaneously have been used to fuse different object detectors~\cite{chari2015pairwise} and for multi-camera MOT~\cite{hofmann2013hypergraphs,leal2012branch}. 
The drawback of these approaches is that they cannot integrate long range information, in contrast to our proposed formulation.
}


\myparagraph{Other combinatorial approaches to MOT.}

The minimum cost arborescence problem, an extension of minimum spanning tree to directed graphs, has been used for MOT in~\cite{henschel2014efficient}.
%
In~\cite{keuper2016multi,keuper2018motion,kumar2014multiple,ristani2014tracking,tang2015subgraph,tang2016multi} the multicut problem has been used for MOT and in~\cite{babaee2018multiple,tang2017multiple} additionally lifted edges have been used to better model long range temporal interactions.
%
The maximum clique problem, which corresponds to multicut with complete graphs has been applied for MOT in~\cite{zamir2012gmcp,dehghan2015gmmcp}.
Maximum independent set, which corresponds to maximum clique on the complement graph, has been used for MOT in~\cite{brendel2011multiobject}.
%
The multigraph-matching problem, a generalization of the graph matching problem, has been applied to MOT in~\cite{hu2019dual}.
Consistency of individual matched detections is ensured by cycle-consistency constraints coming from the multi-graph matching.
%
The works~\cite{Henschel_2018_CVPR_Workshops,henschel2016tracking} reformulate tracking multiple objects with long temporal interactions as a binary quadratic program. 
%If the problem size is small, the optimization problem can be solved optimally by reformulating it to an equivalent binary linear program \cite{henschel2020simultaneous,von2018recovering}. 
For large instances, an approximation is necessary.  

To this end, a specialized non-convex Frank-Wolfe method can be used \cite{Henschel_2018_CVPR_Workshops}.
%
Common to the above state of the art trackers is that they either employ heuristic solvers or are limited in the integration of long range information, in contrast to our work.


\myparagraph{Contribution w.r.t.\ existing combinatorial approaches.}
It is widely acknowledged that one crucial ingredient for obtaining high-quality MOT results is to incorporate long range temporal information to re-identify detections and prevent id-switches.
However, from a theoretical perspective, we believe that long range information has not yet been incorporated satisfactorily in optimization formulations for the data association step in MOT.

In comparison to lifted multicut for MOT, we argue that from the modelling point of view, network flow has advantages.
In multicut, clusters can be arbitrary, while in MOT, tracks are clusters that may not contain multiple detection hypotheses of distinct objects at the same time point.
This exclusion constraint must be enforced in multicut explicitly via soft constraints, while the disjoint paths substructure automatically takes care of it.
On the other hand, the lifted multicut approach~\cite{tang2017multiple} has used the possibility to cluster multiple detections in one time frame.
This directly incorporates non-maxima suppression in the optimization, which however increases computational complexity.

From a mathematical perspective, naively using polyhedral results from multicut is also not satisfactory.
Specifically, one could naively obtain a polyhedral relaxation for the lifted disjoint paths problem by reusing the known polyhedral structure of lifted multicut~\cite{hornakova2017analysis} and additionally adding network flow constraints for the disjoint paths substructure.
However, this would give a suboptimal polyhedral relaxation. 
We show in Section~\ref{sec:constraints} that the underlying structure of the disjoint paths problem can be used to derive new and tighter constraints for lifted edges.
This enables us to use a global optimization approach for MOT.
To our knowledge, our work is the first one to combine global optimization with long range interactions for MOT.



In comparison to works that propose non-convex algorithms or other heuristics for incorporating long range temporal edges~\cite{Henschel_2018_CVPR_Workshops,hu2019dual,zamir2012gmcp,dehghan2015gmmcp} our approach yields a more principled approach and globally optimal optimization solutions via LP-based branch and bound algorithms.




% \myparagraph{Other data association approaches for MOT.}

% \begin{itemize}
%     \item Shortly mention Bells and Whistles \cite{bergmann2019tracking} and CenterTrack \cite{zhou2020tracking}. They effectively recovers missing detections but employs a greedy (Bells and Whistles) and limited (CenterTrack frame-to-frame)  data association strategy, thus being prone to ID switches and suffer from long-term occlusions. Applying BnW to a sequence builds the basis for our tracker. 
%     \item Learning a neural solver \cite{braso2020learning}. Long term information are implicitly processed via graph message passing. Allows to learn features "directly" for the tracking task.
%     Disadvantages:
%     \begin{itemize}
%         \item Memory and computationally demanding as big neural network architecture is employed, modeling the input sequence (subsampling necessary).
%         \item Not directly optimizing tracking problem: Data association not enforced by the neural network (rounding necessary and flow conservation constraint not ensured). 
%     \end{itemize}
%     \item Multicut
%     \begin{itemize}
%         \item In principle. we can use most parts similiar to Lift section about MC
%         \item However, we cannot argue that the MC works employ heuristics in contrast to this work. 
%         \item NEW: \textit{A Two-Stage Minimum Cost Multicut Approach to Self-Supervised Multiple Person Tracking}
%         \begin{itemize}
%             \item Learns pairwise features on the tracking result (cluster short tracks via MC, then update pairwise features, cluster again and iterate).
%             \item Avoids the necessity to create labels for training data. 
%             \item Could be mentioned together with MC approaches.
%         \end{itemize}
%     \end{itemize}
% \end{itemize}


\end{comment}


==> lifted disjoint paths message passing/runtimeTableMOT20-1.tex <==
\begin{center}
\begin{table}
\def\arraystretch{0.8}
\small{
\caption{Runtime and IDF1 comparison of LDP solvers: ApLift (ours)  with 6, 11, 31 and 51 iterations and LifT\cite{hornakova2020lifted} (two step procedure) on first $n$ frames of sequence \textit{MOT20-01} from MOT20.}
\label{tabel:runtime}

\begin{tabular}{c l c c c c c}
%\cline{1-7}
\toprule

$n$ & Measure      & LifT & Our6 & Our11 & Our31 & Our51   \\ \toprule
%\cline{1-7}
%\multirow{2}{*}{30}     & IDF1         & 84.6 & 85.2   & 85.2    & 85.2    & 85.2   \\ % &  &  \\ %\cline{1-7}
%     & time {[}s{]} & 38   & 0      & 1       & 3       & 6    \\ \midrule%   &  &  \\ \cline{1-7}
\multirow{2}{*}{50}     & IDF1$\uparrow$         & $80.6$ & $\mathbf{83.3}$   & $\mathbf{83.3}$    & $81.5$    & $81.5$   \\ % &  &  \\ %\cline{1-7}
     & time {[}s{]} & 272  & 2      & 4       & 16      & 35     \\ \midrule% &  &  \\ \cline{1-7}
%\multirow{2}{*}{75}     & IDF1         & 79.4 & 82.6   & 82.6    & 81.5    & 81.5   \\ % &  &  \\ %\cline{1-7}
%     & time {[}s{]} & 396  & 8      & 14      & 53      & 121    \\ \midrule% &  &  \\ \cline{1-7}
\multirow{2}{*}{100}    & IDF1$\uparrow$         & $80.4$ & $\mathbf{82.5}$   & $\mathbf{82.5}$    & $81.6$    & $81.6$   \\ % &  &  \\ %\cline{1-7}
    & time {[}s{]} & $484$  & $14$     & $24$      & $97$      & $218$    \\ \midrule% &  &  \\ \cline{1-7}
\multirow{2}{*}{150}    & IDF1$\uparrow$         & $78.1$ & $\mathbf{81.0}$   & $\mathbf{81.0}$    & $79.8$    &$ 79.8$   \\ % &  &  \\ %\cline{1-7}
    & time {[}s{]} & $1058$ & $25$     & $46$      & $192$     & $431$    \\ \midrule% &  &  \\ \cline{1-7}
\multirow{2}{*}{200}    & IDF1$\uparrow$         & $73.2$ & $\mathbf{75.4}$   & $\mathbf{75.4}$    & $74.6$    & $74.6$  \\ %  &  &  \\ %\cline{1-7}
    & time {[}s{]} &  $2807$ & $36 $    & $66$      & $277$     & $616$   \\ \bottomrule% &  &  \\ \cline{1-7}
\end{tabular}
}
\vspace{-5.2mm}
\end{table}
\end{center}

==> lifted disjoint paths message passing/runtimeTableMOT20-2.tex <==
\begin{table}[h]
\small{
%\caption{LDP solver runtime and IDF1 comparison between our solver with 6, 11, 31 and 51 iterations against two-step
%Lif\_T\cite{hornakova2020lifted} on first $n$ frames of sequence \textit{MOT20-02} from MOT20.}
\caption{Runtime and IDF1 comparison of LDP solvers: ApLift (ours)  with 6, 11, 31 and 51 iterations and LifT\cite{hornakova2020lifted} (two step procedure) on first $n$ frames of sequence \textit{MOT20-01} from MOT20.}
\label{tabel:runtime02}

\begin{tabular}{c l c c c c c}
%\cline{1-7}
\toprule

$n$ & Measure      & LifT & Our6 & Our11 & Our31 & Our51   \\ \toprule
%\cline{1-7}
%\multirow{2}{*}{30}     & IDF1         & 84.6 & 85.2   & 85.2    & 85.2    & 85.2   \\ % &  &  \\ %\cline{1-7}
%     & time {[}s{]} & 38   & 0      & 1       & 3       & 6    \\ \midrule%   &  &  \\ \cline{1-7}
\multirow{2}{*}{50}     & IDF1$\uparrow$         & $\mathbf{83.4}$ &  $\mathbf{83.4}$   &  $\mathbf{83.4}$    &  $\mathbf{83.4}$    &  $\mathbf{83.4}$   \\ % &  &  \\ %\cline{1-7}
     & time {[}s{]} & $62$  & $4$      &$ 7$       & $25$      & $46$     \\ \midrule% &  &  \\ \cline{1-7}
%\multirow{2}{*}{75}     & IDF1         & 79.4 & 82.6   & 82.6    & 81.5    & 81.5   \\ % &  &  \\ %\cline{1-7}
%     & time {[}s{]} & 396  & 8      & 14      & 53      & 121    \\ \midrule% &  &  \\ \cline{1-7}
\multirow{2}{*}{100}    & IDF1$\uparrow$         & $\mathbf{80.6}$ & $79.9$   & $79.9$    & $79.9$    & $79.9$   \\ % &  &  \\ %\cline{1-7}
    & time {[}s{]} & $124$  & $30$     &$ 54$      & $182$      & $360$    \\ \midrule% &  &  \\ \cline{1-7}
\multirow{2}{*}{150}    & IDF1$\uparrow$         & $\mathbf{78.7}$ & $76.8$   & $76.8$    & $76.8$    & $76.8$   \\ % &  &  \\ %\cline{1-7}
    & time {[}s{]} & $222$ & $61$     & $110$      & $378$     & $780$    \\ \midrule% &  &  \\ \cline{1-7}
\multirow{2}{*}{200}    & IDF1$\uparrow$         & $\mathbf{77.6}$& $75.8$   & $75.8$    & $75.8$    & $75.8$  \\ %  &  &  \\ %\cline{1-7}
    & time {[}s{]} & $354$ & $95$     & $177$      & $604$     & $1195$   \\ \bottomrule% &  &  \\ \cline{1-7}
\end{tabular}
}
\end{table}
